SinClave: Hardware-assisted Singletons for TEEs

For trusted execution environments (TEEs), remote attestation permits establishing trust in software executed on a remote host. It requires that the measurement of a remote TEE is both complete and fresh: We need to measure all aspects that might determine the behavior of an application, and this measurement has to be reasonably fresh. Performing measurements only at the start of a TEE simplifies the attestation but enables "reuse" attacks of enclaves. We demonstrate how to perform such reuse attacks for different TEE frameworks. We also show how to address this issue by enforcing freshness - through the concept of a singleton enclave - and completeness of the measurements. Completeness of measurements is not trivial since the secrets provisioned to an enclave and the content of the filesystem can both affect the behavior of the software, i.e., can be used to mount reuse attacks. We present mechanisms to include measurements of these two components in the remote attestation. Our evaluation based on real-world applications shows that our approach incurs only negligible overhead ranging from 1.03% to 13.2%.

==> shepherd_version/00_abstract.tex <==
\begin{abstract}
For trusted execution environments (TEEs), remote attestation permits establishing trust in software executed on a remote host.
It requires that the measurement of a remote TEE is both complete and fresh:
We need to measure all aspects that might determine the behavior of an application, and this measurement has to be reasonably fresh.
Performing measurements only at the start of a TEE simplifies the attestation but enables ``reuse'' attacks of enclaves.
We demonstrate how to perform such reuse attacks for different TEE frameworks. We also show how to address this issue by enforcing freshness -- through the concept of a singleton enclave -- and completeness of the measurements. 
Completeness of measurements is not trivial since the secrets provisioned to an enclave and the filesystem's content can both affect the software's behaviour, \ie{}, can be used to mount reuse attacks.
We present mechanisms to include measurements of these two components in the remote attestation. Our evaluation based on real-world applications shows that our approach incurs only negligible overhead, ranging from $1.03$\% to $13.2$\%.



% For trusted execution environments (TEEs), remote attestation permits to establish trust into software executed in a remote host. 
% However, the assumption, that the measurement of TEEs can describe the behavior of this software, is misleading. It only guarantees software integrity before it runs. 
% We show that one needs to balance the need for software configuration at runtime and trust in the execution environment. 
% This flexibility can lead to the exploitation of a loophole in remote attestation, allowing an attacker to steal private software’s configuration and secrets. 

% In this paper, we first provide insight into a vulnerability in remote attestation and then design and implement a protection mechanism, called \sys. 
% \sys strengthens the measurement of TEEs by introducing the concept of singleton TEEs that, in combination with security policies and rejuvenation, provide both the flexibility for software configuration and strong security guarantees. 
% According to our best knowledge, we are the first to detail these shortcomings in remote attestation for legacy applications and also to provide a solution to it. 
% Our evaluation based on real-world applications shows that \sys incurs only negligible overhead.


	
% \rk{The abstract should mention that our solution provides both freshness and completeness with regard to attestation. We need to say that both are important for use cases such as OpenVino where dynamic data is loaded after typical attestation occurs. Providing a use case such as OpenVino with a problem is essenitial.}

% \rk{The abstract should state that our solution imposes only acceptable overhead (with numbers)}




%Intel Software Guard Extensions (SGX) recently has been widely adopted in clouds since its ability to protect code and data of application during computation. SGX offers an isolated secure memory area called enclaves, where the code and data can be executed safely.  Besides that, it supports also another important feature called remote attestation that allows users to verify the integrity of their applications running inside SGX enclaves in remote hosts.
%
%In this paper, we report a serious vulnerability of this remote attestation mechanism by presenting a novel exploitation technique to bypass it. We demonstrate this attack in popular SGX frameworks, e.g., SGX-LKL and in the Microsoft Azure Attestation (MAA) system of Microsoft.
%In addition to that, we also provide a protection mechanism against this attack and integrate it into a configuration and attestation framework. Our evaluation results show that our protection mechanism can defend against the attack with negligible overhead.
\end{abstract}


==> shepherd_version/01_introduction-big_picture.tex <==
\section{Introduction}

\fg{
    TODO: We must point out that we are interested in supporting legacy applications in SGX.
    This is a given for use but the reader may not expect it.
    Further, it is important later on such that we can argue, or rather justify, why SCONE and SGX-LKL chose a very flexible approach for enclave measuring.
    Mention Lift and Shift.

    Bigger Picture Motivation:
    % IDEA: lift and shift of existing applications into TEE is awesome
    % however, if we do this we should use SGX as TEE since it offers significantly better security
    Moving legacy software into \glspl{tee} is a promising prospect for significantly improving the security of existing applications and to make them fit to run under stringent privacy regulations, such as the EU's GDPR with minimal effort for the user.
    \gls{sgx} is arguably the more secure \gls{tee} technology compared techniques where an entire \gls{os} must be trusted (AMDSEV SNP, TDX, TrustZone, ...).
    While with \gls{sgx} only the program and an additional supporting code allowing the legacy program to seamlessly run inside of \gls{sgx} must be trusted yielding a significantly smaller \gls{tcb}.

    % IDEA: lots of works about how to run legacy software in SGX (TODO: add references of the most important works)
    This prospect lead to efforts to overcome factors limiting the use of \gls{sgx} to protect legacy software and lead to solutions we refer to as \gls{sgx} frameworks.
    For the mere functioning of legacy software inside of \gls{sgx} the frameworks must already solve a bunch of challenges: the system call instruction is not available inside of \gls{sgx}, memory management must be done independently of the \gls{os}, OTHER CHALLENGES.
    Many of these solution introduce significant performance penalities compared to native execution which is evident as most techniques there're replacing have been optimized for years. 
    Therefore, \gls{sgx} frameworks introduce their own optimizations.
    Most notably, SCONE was the first framework that used what is now known as switchless system calls improving system call performance.
    Recently, Occlum reported even better performance by combining switchless system calls with the recent IO-uring asynchronous system call mechanism.

    % IDEA: but securing these naive applications is also hard and less work went into this
    % most well known is shielding, but 
    Apart from the functionality additional security guarantees must be added by the \gls{sgx} framework to protect the legacy software.
    After all, the legacy software was developed for a less strict threat-model where the system is trusted.
    When executed inside of \gls{sgx}, the framework must protected the naive applications from the now untrusted system.
    This is done through shielding~\cite{haven} where interaction with the \gls{os} is sanitized, and data is protected, by the \gls{sgx} framework.
    A typical example for this is the file system where \gls{sgx} frameworks transparently encrypt file content before it is handed to the \gls{os} for persisting and integrity is verified when files are read.
    
    Last but not least, deployment of applications becomes significantly more complicated with \gls{tee} since configuration data containing secrets and keys must never be visible to the untrusted system.
    For this challenge, at least two frameworks (SCONE~\cite{palaemon} and SGX-LKL~\cite{sgx-lkl}) provide an integrated solution in which the legacy's applications configuration interfaces are served transparently after the verifier ensured themselves that the remote \gls{tee} was not tampered.
    Other frameworks we're aware of only provide the building blocks, but require the user to implement secure provisioning by themselves which contradicts the notion of legacy applications.

    In this work we investigate current \gls{sgx} frameworks under the aspect of legacy applications compatibility.
    In particular, we focus on the aspect of trust establishment, that is (remote) attestation.
    We found that existing solution either are too restrictive for many legacy applications or fail to protect the secrets of dynamic programs, in particular, language interpreters.
    We noticed that the lack of a suitable solution is due to the inherent design decisions in the attestation of \gls{sgx} that simple ad-hoc solution are unable to compensate.
    Precisely, the trusted information a verifier obtains during attestation does not change throughout the entire lifetime of an enclave, while the enclave can engage into attestation arbitrarily often.
    We will show how these aspects enable an adversary to impersonate a fresh enclave to obtain secrets during configuration provisioning under certain conditions.
    We introduce singleton enclaves that have unique enclave measurements to mitigate such attacks and enable the necessary flexibility needed by legacy applications.
}

In the last years, \glspl{tee} technologies, such as Intel SGX, have gained much attention industry~\cite{AzureSGX, IBMCloudSGX} as well as in academia~\cite{arnautov2016scone,costan2016intel,tsai2017graphene,shen2020occlum} since their ability to protect cloud-native applications (including code and data) not only at rest, in transit, but also during computations (``in use''), against powerful attackers with privileges accesses to the underlying system software (e.g., operating system and hypervisor). 
To ensure confidentiality and integrity of applications, TEEs execute their code and data inside an encrypted memory region called \emph{ enclave}. 
Adversaries with privileges accesses cannot interfere the memory region and only CPU hardware can decrypt and execute the application inside the enclave.  

Besides the ability to run applications inside enclaves, TEEs also, provide another key feature namely \emph{Remote Attestation}~\cite{costan2016intel} which allows users to verify the trustworthiness of the application inside enclaves running on a remote host. Remote attestation provides for users certain guarantees about remote enclaves before transferring secrets for their applications running insides the enclaves, i.e.,  applications are not modified by anyone (e.g., an attacker).

While TEEs such as Intel SGX have been adopted in practice~\cite{AzureSGX,IBMCloudSGX}, researchers recently demonstrated that TEEs  are vulnerable to side-channel attacks~\cite{Kocher2018spectre, chen2018sgxpectre, Foreshadow, Lipp2018meltdown}. To mitigate these attacks, protection mechanisms have been proposed~\cite{DRSGX, oblivious-ram2, oblivious-ram1, cloak,  raccoon, szefer_cache_attacks}. Intel has been also working to release various patches, microcode updates to mitigate SGX side-channel attacks.
In this paper, we however turn our focus to the second key feature of TEEs which is the \emph{ remote attestation} mechanism.  We present an attack that bypasses the remote attestation protocol. This attack does not require attacking the sealing mechanism of TEEs as the previous work~\cite{van2020sgaxe}.  We demonstrate a detailed attack on Intel SGX remote attestation because Intel SGX is widely used in practice. 
This attack is a serious problem since the remote attestation typically is the first step of TEE users need to perform to make sure their application inside enclaves on a remote host running correct code, data and the enclaves were initialized correctly with genuine hardware. Thereafter, the users establish secure connections to the enclaves to transfer secrets and configuration. Thus, if an attacker can bypass the remote attestation, she can read and steal all secrets of the application running inside enclaves as well secrets of TEE provider used for performing the attestation. 

%\dodo{need to rewrite}
This attack is based on the fact that almost all applications dynamically load libraries and their configuration during runtime. This gives an attacker a chance to add malicious code into libraries or manipulate the configuration which are loaded into enclaves, then she can steel secrets of applications and bypass the remote attestation. The remote attestation mechanism of TEEs just attests to the integrity of an application right before running but not during its runtime. Thus, applications with the pre-compiled binaries (e.g., Python interpreter) are seriously vulnerable to this attack since their behavior is determined through their configuration.

%Indeed, \gls{sgx}' attestation mechanism combined with pre-compiled binaries, e.g., Python interpreter introduce a significant security risk if the program's behavior is significantly determined through its configuration.
%The reason is that  in \gls{sgx} the software identity that is attested is only calculated based on the enclave's code.
%Following this observation we distinguish a program's code to be everything that is loaded into the enclave's memory influencing its software identity.
%Any other data that influences the programs behavior is regarded as configuration.
%These might be configuration files, shared objects only loaded at program runtime, or source or byte code files.
%Lastly, there is program data.
%
%Applications written in interpreted languages are a prime example for programs whose behavior is determined through configuration.
%Their program code consists of their interpreters whereas their behavior is determined by source or byte code files that are read at runtime by the interpreter.

%{\bf Attack overview.}
Let us present an overview of this attack by giving a real-world scenario. Imagine a service provider who wants to run a Python application securely in a \gls{tee} in the cloud.
We assume the Python interpreter can be executed securely in the \gls{tee}, in the case of \gls{sgx}, for example by using frameworks such as SCONE~\cite{arnautov2016scone}, SGX-LKL~\cite{priebe2019sgx}, or Graphene-SGX~\cite{tsai2017graphene}.
The service provider triggers the application's cloud deployment and subsequently uses remote attestation to assure the \gls{tee} was constructed without manipulations before securely sending the application's secrets.
The attacker can observe and intercept this attestation process as follows. %The adversary observed and intercepted this actions.
She starts the requested Python interpreter correctly in the \gls{tee}, but configures it in a such way that it will load a malicious library to execute a \gls{tee} impersonator program. 
%This is straight forward as an interpreter the \gls{tee}'s whole behavior is configuration dependant.

\rk{The approach of secret-provisioning an application after attestation is specific to Scone, right? However at this point the reader doesn't know anything about secret provisioning.}
\rk{Needs to be introduced.}
\rk{Secret provisioning after attestation needs to be introduced.}
This impersonator program then will engage in the remote attestation procedure with the service provider and obtain his secrets for the Python application.
The service provider is not able to detect this manipulation since the attestation procedure only captures the \gls{tee}'s initial state with which the attacker did not tamper.

Vulnerabilities in a program's configuration handling code that is typically not considered as a vector of attack can make any program exploitable by the re-attestation attack. 
%We believe that state-of-the-art solutions are inadequate for practical systems.
Considering this attack, Haven~\cite{baumann2015shielding} proposed to incorporate its configuration into the \gls{tee} such that the attestation would also reflect the configuration.
This would prevent the re-attestation attack by making the attackers manipulation visible through the attestation procedure but it would also reveal the \gls{tee}'s configuration and, thus, its secrets.
Integrating the service provider's cryptographic identity into the \gls{tee} and enforcing that it would only start with configurations signed with this identity would prevent the attacker from configuring the \gls{tee}.
Unfortunately, it would also decrease the usability of the system as every \gls{tee} would need to be individualized which prohibits established procedures for software distribution and deployment.
In this paper, we overcome this issue by proposing a novel protection mechanism against this attack that does not break the usability of legacy applications and incur only a negligible overhead. 

The contributions of this paper are as follows: %\fg{add section references}
\begin{itemize}
    \item We illustrate a practical attack on \gls{tee} secret provisioning subverting all \gls{tee} protection goals (\(\S\)\ref{sec:attack}).
    \item We show the novelty of our attack by exploiting state-of-the-art \gls{tee} runtime systems (\(\S\)\ref{sec:framework-attack}). %showing that even ad-hoc solutions are not present.
    \item We highlight a previously neglected vector of attack for \gls{tee} software that renders the majority of system vulnerable to the presented attack (\(\S\)\ref{sec:attack-discussion}).
    \item We propose, implement and evaluate a new secret provisioning mechanism that prevents the presented attack and does not prohibit a \gls{cots} software distribution model. 
    Our protection mechanism is flexible since it supports the change of input files, arguments, environment variables, etc required to run typical applications as well as software updates (\(\S\)\ref{sec:protection}).
    \item We conduct micro- macro-benchmarks to demonstrate that our protection mechanisms incur only negligible overhead and can be used in practice (\(\S\)\ref{sec:evaluation}). 
\end{itemize}





==> shepherd_version/01_introduction.tex <==
\section{Introduction}

%\fg{
%    TODO: We must point out that we are interested in supporting legacy applications in SGX.
%    This is a given for use but the reader may not expect it.
%    Further, it is important later on such that we can argue, or rather justify, why SCONE and SGX-LKL chose a very flexible approach for enclave measuring.
%    Mention Lift and Shift.
%}

\gls{tee} technologies, such as Intel \gls{sgx}, have gained much attention in the industry~\cite{AzureSGX, IBMCloudSGX} as well as in academia~\cite{arnautov2016scone, sgx-explained, tsai2017graphene, shen2020occlum}.
\glspl{tee} can protect cloud-native applications (code and data) not only at rest, in transit, but also during computation (in use) against powerful attackers with privileged access to the underlying system software (\eg{}, the operating system or the hypervisor), as well as, hardware.
To ensure confidentiality and integrity of applications, \glspl{tee} execute their code and data inside an encrypted memory region called \emph{enclave}. 
Adversaries with privileged access cannot read or interfere with the memory region and only the processor can decrypt and execute the application inside an enclave.  

Various hardware-assisted \glspl{tee} exist today, \eg{}, Intel SGX~\cite{Anati2013a,McKeen2013}, ARM TrustZone~\cite{TrustZone},  AMD SEV SNP~\cite{AMD-SEV-SNP}, and Intel TDX~\cite{TDX}.
Out of these \glspl{tee}, Intel SGX has been widely adopted in practice~\cite{AzureSGX, IBMCloudSGX} since 2015.
It enables a general-purpose \emph{ring 3}-enabled TEE and yields a significantly smaller \gls{tcb} in comparison with other solutions where typically a whole \gls{os} is part of the \gls{tcb}.
Furthermore, running legacy applications without source code changes is supported by several SGX platforms~\cite{arnautov2016scone, priebe2019sgx, tsai2017graphene, shen2020occlum}.

Arguably, just executing legacy applications in Intel SGX environments is not enough to ensure strong security guarantees.
First, the legacy applications were developed for a weaker threat model that trusts the underlying system software.
Thus, the \gls{sgx} frameworks must employ additional protection mechanisms to protect the naive legacy application against the elevated threats in the \gls{sgx} threat model.
An example is the file system for which \gls{sgx} frameworks transparently encrypt file content before it is persisted by the \gls{os}.
The content's integrity is additionally verified when files are read.
Second, deployment of legacy applications becomes significantly more complicated in \glspl{tee} as configuration data (containing secrets) for these applications must be hidden from potentially malicious system software.

To handle these problems, \gls{sgx} frameworks, such as Gra\-phe\-ne-SGX~\cite{tsai2017graphene} or Occlum~\cite{shen2020occlum}, only provide the building blocks for users and require individual implementation of secure data provisioning.
This approach contradicts the common goal to \emph{support legacy applications} without changing their source code.
Other frameworks, \eg{}, SCONE~\cite{palaemon,arnautov2016scone} and SGX-LKL \cite{priebe2019sgx}, provide an integrated solution that 
transparently serves software configurations only after it was verified that the application is not modified and the \gls{tee} is genuine. %and that an adversary did not alter the application.

The verification process is called \emph{Remote Attestation}~\cite{sgx-explained} and allows one to establish trust in the application running inside an enclave on a remote host.
%Remote attestation provides for users certain guarantees about remote enclaves before transferring secrets for their applications running insides the enclaves, i.e., applications are not modified by anyone (e.g., an attacker).
Remote attestation is a first step one performs to ensure that an application on a remote host, runs the correct code inside a genuine hardware enclave and it was initialized correctly.
After that, users establish a secure connection to the enclave to transfer secrets and configuration to their application.

We show that current remote attestation mechanisms for \glspl{tee}, \eg{}, Intel SGX, struggle to provide the expected trust and present an attack that bypasses the remote attestation protocol.
We further establish that the measurement during attestation needs to be both \textit{complete}, \ie{}, measure all aspects that determine the behavior, and \textit{fresh}, \ie{}, the measurement reflects the current behavior.
During runtime, applications may load libraries or open shared volumes, which may change the behavior.
The measurement should reflect the dynamic behavior, and ensure the freshness (to protect against ``reuse'' attacks), of the legacy applications running inside enclaves.
%This additional data might determine the behavior of applications or even corrupt them. 
%In consequence, the measurement for the attestation has to be complete and fresh to include dynamically loaded data during runtime.

Unfortunately, performing measurements with current attestation mechanisms of TEEs only ensures an application's  integrity at the starting of an enclave.
Thus, it's vulnerable to ``reuse'' attacks, as we show in \S{}\ref{sec:attack}: one can use a previous measurement to impersonate a TEE with a different expected behavior.
The vulnerability is based on the fact that almost all applications dynamically load data, libraries, and configurations during runtime, which can change their behavior.
%\rk{
%Insert OpenVino example here.
%Introduction needs use openvino and volumes as example usecase.
%Pointing at dynamic data (volumes beeing mounted) in addition to application configuration gives the story more strength.
%}
An attacker adds malicious code via libraries or manipulates the configuration loaded into enclaves or loads data that might trigger some application bug. 
They can then steal secrets of an application by bypassing the remote attestation as sketched in the following example.

%While TEEs such as Intel SGX have been adopted in practice~\cite{AzureSGX,IBMCloudSGX}, researchers recently demonstrated that TEEs  are vulnerable to side-channel attacks~\cite{Kocher2018spectre, chen2018sgxpectre, Foreshadow, Lipp2018meltdown}. To mitigate these attacks, protection mechanisms have been proposed~\cite{DRSGX, oblivious-ram2, oblivious-ram1, cloak,  raccoon, szefer_cache_attacks}. Intel has been also working to release various patches, microcode updates to mitigate SGX side-channel attacks.
%In this paper, we however turn our focus to the second key feature of TEEs which is the \emph{ remote attestation} mechanism.  We present an attack that bypasses the remote attestation protocol. This attack does not require attacking the sealing mechanism of TEEs as the previous work~\cite{van2020sgaxe}.  We demonstrate a detailed attack on Intel SGX remote attestation because Intel SGX is widely used in practice. 
%\dodo{need to rewrite}

%Indeed, \gls{sgx}' attestation mechanism combined with pre-compiled binaries, e.g., Python interpreter introduce a significant security risk if the program's behavior is significantly determined through its configuration.
%The reason is that  in \gls{sgx} the software identity that is attested is only calculated based on the enclave's code.
%Following this observation we distinguish a program's code to be everything that is loaded into the enclave's memory influencing its software identity.
%Any other data that influences the programs behavior is regarded as configuration.
%These might be configuration files, shared objects only loaded at program runtime, or source or byte code files.
%Lastly, there is program data.
%
%Applications written in interpreted languages are a prime example for programs whose behavior is determined through configuration.
%Their program code consists of their interpreters whereas their behavior is determined by source or byte code files that are read at runtime by the interpreter.


% Applications with the pre-compiled binaries (e.g., Python interpreter) are vulnerable to this attack since their behavior is determined through their configuration, \eg{} the Python script, and because the remote attestation mechanism of TEEs just attests to the integrity of an application right before running but not during its runtime.

Imagine a service provider (i.e., cloud user) who wants to run a Python application securely in a \gls{tee} in the cloud, \eg{}, an AI application based on PyTorch or TensorFlow. 
%We assume the Python interpreter can be executed securely in the \gls{tee}, in the case of \gls{sgx}, for example by using frameworks such as SCONE~\cite{arnautov2016scone} or SGX-LKL~\cite{priebe2019sgx}.
The service provider triggers the application's cloud deployment and subsequently uses remote attestation to assure the \gls{tee} was constructed without manipulations before securely sending the application's secrets.
The attacker can observe and intercept this attestation process by starting the requested Python interpreter correctly in the \gls{tee}, but configuring it such that it will load a malicious library to execute a \gls{tee} impersonator program. 
%This is straight forward as an interpreter the \gls{tee}'s whole behavior is configuration dependant.
This impersonator program then will correctly engage in the remote attestation procedure with the service provider and obtain his secrets for the Python application.
The service provider cannot detect this manipulation since the attestation procedure only captures the \gls{tee}'s initial state which the attacker did not alter.

Vulnerabilities in a program's configuration handling code -- typically not considered a vector of attack -- can make any program exploitable to the ``reuse'' attack. 
%We believe that state-of-the-art solutions are inadequate for practical systems.
Considering this attack, Haven~\cite{baumann2015shielding} proposed to incorporate configurations into the \gls{tee} such that the attestation would also include them.
%prevents the re-attestation attack by making the attackers manipulation visible through the attestation procedure but it
However, this would also reveal the \gls{tee}'s configuration and, thus, its secrets.
An alternative solution integrates the service provider's cryptographic identity into the \gls{tee} and enforces that the application would only start with correctly signed configurations.
% signed with this identity would prevent the attacker from configuring the \gls{tee}.
This approach decreases the system's usability as every \gls{tee} needs to be individualized, prohibiting established procedures for software distribution and deployment.

We overcome the portrayed issues by proposing a novel protection mechanism against ``reuse'' attacks on remote attestation.
Our solution does not break the usability of legacy applications, \eg{}, supporting secure dynamic configuration and secure mounting of volumes, and incurs only a negligible overhead. 
%
Our contributions are as follows: %\fg{add section references}
\vspace{-5mm}
\begin{itemize}
    \item We comprehensively describe remote attestation in TEEs, especially Intel SGX (\S{}\ref{subsec:intel-sgx-remote-attestation} and \S{}\ref{sec:attestation}).
    \item We illustrate a practical attack on \gls{tee} secret provisioning, subverting all \gls{tee} protection goals (\S{}\ref{sec:attack}).
    \item We highlight a previously neglected vector of attack for \gls{tee} software rendering most systems vulnerable to the presented attack (\S{}\ref{sec:attack}).
    \item We show the novelty of our attack by exploiting state-of-the-art \gls{tee} runtime systems (\S{}\ref{sec:attack_overview}). %showing that even ad-hoc solutions are not present.
    \item We implement and evaluate a new flexible secret provisioning mechanism preventing the presented attack while supporting changes of input files, arguments, environment files, etc., as well as software updates (\S{}\ref{sec:protection}).
    %while not prohibiting a \gls{cots} software distribution model
    \item We conduct micro- and macro-benchmarks to demonstrate that our protection mechanisms incur only negligible overhead and can be used in practice (\S{}\ref{sec:evaluation}). 
\end{itemize}
% \vspace{5mm}


==> shepherd_version/02_background.tex <==
\section{Background}\label{sec:background}

\subsection{Trusted Execution Environments}
Trusted Execution Environments (TEEs), such as ARM TrustZone \cite{TrustZone}, AMD SEV SNP~\cite{AMD-SEV-SNP}, Intel SGX~\cite{AzureSGX, sgx-explained}, and Intel TDX~\cite{TDX}, support the design of complex, yet secure, applications.
A \gls{tee} is a tamper-resistant processing environment that guarantees the authenticity, the integrity and the confidentiality of its executing code, data and runtime states (e.g., CPU registers, memory and sensitive I/O).
The content of \gls{tee} remains resistant against software attacks even from privileged code, as well as any physical attacks performed on the main memory of the system.
In addition, \glspl{tee} offer \emph{attestation} for proving their trustworthiness to third-parties.
However, we demonstrate the vulnerability of remote attestation by demonstrating a serious ``reuse'' attack on the \gls{tee} of Intel \gls{sgx} (\S{}\ref{sec:attack}).
%Intel SGX has appeared as the most widely adopted TEE~\cite{AzureSGX,IBMCloudSGX} in practice.
%This attack can affect running services in production which leverage Intel SGX for confidential computing~\cite{confidential-computing}.\rk{Which paper is meant here?}
We also introduce a mechanism to protect against this attack in practice (see \S{}\ref{sec:protection}).



==> shepherd_version/02_background_intel_sgx.tex <==
\subsection{Intel SGX Security Argument}
\label{subsec:intel-sgx-remote-attestation}

Before introducing the attack that bypasses remote attestation, we describe the technical building blocks that our work builds upon.
These are primarily the \gls{sgx} enclave creation, measurement and attestation procedures.
Enclave measurement and attestation are implemented mostly in hardware, so users cannot modify them.
Therefore, we have to rely on existing functionality to establish a practical solution usable with current hardware.
In the following, we will explain the fundamentals of the security argument for attestation in \gls{sgx} and show how existing frameworks use \gls{sgx} attestation and the resulting ramifications.
We further introduce the concepts for validating that an enclave has not been tampered with before its initialization.
We omit aspects of \gls{sgx} that are superfluous for the understanding of this work and that have been sufficiently explained elsewhere~\cite{sgx-explained}.


\emph{Enclave verification} begins with the creation of the enclave itself:
Representations of each executed operation are hashed into a measurement value (\S{}~\ref{sec:background:enclave_creation} and \S{}~\ref{sec:background:sha-256}).
Enclave creation is finalized with enclave initialization during which signer based verification properties are bound to the enclave (\S{}~\ref{sec:background:enclave_initialization}).
Once initialized an enclave can engage in remote attestation (\S{}~\ref{sec:background:attestation}) to convince the verifier of its integrity.

\subsubsection{Enclave Creation}\label{sec:background:enclave_creation}

\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.5]{figures/sgx_enclave_creation}
    \vspace{2mm}
    \caption{Enclave Creation Procedure.}\label{fig:enclave_creation}
    \Description{No description.}
    
\end{figure}

An \gls{sgx} enclave is created by a program referred to as the \texttt{starter}, which is not part of the \gls{tcb}~\cite{guide2020intel}.
The \texttt{starter} utilizes four \gls{sgx} instructions to create the enclave as shown in Figure~\ref{fig:enclave_creation}.
\texttt{ECREATE} creates an enclave, more precisely, its metadata \gls{secs} and, therefore, determines its maximal size and enclave attributes, such as 64-bit mode, debug mode or whether it requires certain extended processor features such as \gls{avx} or \gls{cet}.
Once the enclave is created, \texttt{EADD} and \texttt{EEXTEND} instructions are used to add each page (4\thinspace{}kB) of code and data to the enclave's memory and extend its measurement respectively. 
Once the enclave's memory is set up, the enclave is initialized with \texttt{EINIT} preventing any further modifications of the enclave from the outside.
In the initialized state the enclave can be entered and assumes control over itself.

\subsubsection{Secure Hash Algorithm 256 (SHA-256)}\label{sec:background:sha-256}

Our solution tightly interacts with the \emph{hash algorithm} used for enclave measurement.
Hence, we provide the necessary details about the utilized SHA-256 algorithm.
SHA-256~\cite{penard2008secure, pub2012secure} is one variant of the Secure Hash Algorithm 2 cryptographic hash functions.
The SHA hash functions are based on Merkle-Damg\r{a}rd construction~\cite{merkle1979secrecy} with Davies-Meyer compression functions.
SHA-256 maintains an internal state of 256-bits that are organized in 8 values (\(H1\) \dots \(H8\)) with 32-bit each that eventually becomes the hash value.
An arbitrary message, whose length is only limited by the hash internal length counter of 64-bit, is compressed into these 8 values.
% Calculating a SHA-256 hash value can be summarized in three steps:  (see Figure~\ref{fig:sha}):

% \emph{Initialization \raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {1}}}}:
% The hash state is initialized with initialization vector values according to the SHA-256 standard.

% \emph{Updating \raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {2}}}}:
% Each 64-byte chunk of message data is processed iteratively with a procedure, we summarize as SHA Round and by updating the length counter.
% The SHA Round consumes the incoming message chunk and intermingles it with the current hash state (\(H1\)\dots{}\(H8\)).
% The output of the SHA Round becomes the new hash state.

% \emph{Finalization \raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {3}}}}:
% After the entire message is consumed through iterative updating, the hash calculation is finalized yielding the hash value.
% For this, the message length counter value is hashed into the hash state using the SHA Round procedure.
% The 64-bit message length is padded according to a standardized padding scheme to fill the entire 64-byte input of the SHA Round.
% This final result of the SHA Round calculation is the SHA-256 hash value of the input message.

% \url{https://qvault.io/cryptography/how-sha-2-works-step-by-step-sha-256/}

Note that, due to the construction of the hash algorithm, for every \(64\) Bytes of compressed input an internal intermediary state is reached that can be described with \(256\) bit of internal hash state and \(64\) bit of already compressed input.
%\footnote{Although, strictly speaking only 58-bit are necessary to described the message length.}
During an \gls{sgx} enclave measurement, each operation's representation is a multiple of \(64\) Bytes in length.
%It follows that, after each enclave construction operation the enclave measurement hash calculation is in a state that can be described as said before.

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.4\textwidth{}]{figures/SHA256-schema}
%     \vspace{2mm}
%     \caption{Schema of SHA256.}\label{fig:sha}
%     \Description{No description.}
% \end{figure}


\subsubsection{Enclave Initialization}\label{sec:background:enclave_initialization}

Before locking the enclave from further modifications, \eg{}, from system software, the enclave initialization verifies the \gls{sigstruct}.
The \gls{sigstruct} is created by the enclave signer, \eg{}, the software owner
and specifies the expected enclave measurement value (\texttt{MRENCLAVE}),
enclave attributes, the signer-assigned product id, and a security version number.
The information is protected by an RSA signature created with the enclave signer's key.
Upon enclave initialization, the processor will ensure that the \gls{sigstruct} has not been manipulated and that the constructed enclave matches it.
To summarize, the \gls{sigstruct} enables the signer to specify the \gls{sgx} configuration for a particular enclave and to specify access to specific \gls{sgx} sealing keys.
The \gls{sgx} \gls{sigstruct} can not prevent manipulations entirely.
As it is handled by system software, the adversary can modify the \gls{sigstruct} and sign it with their own key.\footnote{An adversary may execute an enclave with a configuration not intended by the signer to allow for exploitation.}
Therefore, the signer's identity (\texttt{MRSIGNER}) is incorporated during the attestation procedure. %(detailed next).
%Also it reflects in (some of) the keys the enclave can derive as it participates in the derivation process.

Another mechanism utilized during enclave initialization is the verification of the \gls{einittoken} data structure.
An \gls{einittoken} allows an enclave with a certain \texttt{MRENCLAVE} measurement, \texttt{MRSIGNER} identity, and enclave attributes to start.
It is generated by a dedicated system enclave, the \texttt{launch enclave}, and must be provided to the \texttt{EINIT} instruction initializing the enclave for it to succeed.
In the first implementation of \gls{sgx}, only enclaves signed by Intel were allowed to become launch enclaves.
%~\footnote{Launch enclaves utilize \gls{sgx}' key derivation to obtain the platform's launch key with which the \gls{einittoken} is protected.}\rk{What is \gls{sgx} key derivation?}
The launch enclave from Intel generated \gls{einittoken}s for any enclave in debug mode.
However, enclaves in production mode must be signed with a signer's key that Intel authorizes to obtain a \gls{einittoken} data structure.
%This attracted great criticism from academics~\cite{costan2016intel} and practitioners alike and postponed incorporation of \gls{sgx} into the Linux Kernel~\cite{lwn2019sgx}.
%Addressing this criticism 
Later, Intel introduced \gls{flc}, allowing the platform owner to determine which launch enclaves can run.
With \gls{flc} the default launch enclave allows any enclave to run in production mode.

\subsubsection{Attestation with SGX}\label{sec:background:attestation}

When an enclave is running (initialized and entered) it can request a report from the processor.
The report entails the enclave's \texttt{MRENCLAVE}, \texttt{MRSIGNER}, enclave attributes as well as information about the platform's processor.
With the help of a quoting enclave the report can be transformed into a remotely verifiable quote.
Note that report and quote show the enclaves state at the point of initialization.
That is, any modifications afterwards (by the enclave) are not reflected in the quote and are, thus, not observable by the remote verifier.

Intel has defined protocols for local and remote attestation to be used for verifying the genuineness of an SGX enclave and the software executed within the SGX enclave~\cite{Anati2013a}.
%These protocols have already been described in detail in several publications [\dots].
%Hence, we provide only a summary with the most important information needed in the context of our work.
\gls{sgx}'s attestation scheme relies on a key generation facility and on a provisioning service.
During the manufacturing process, a ``Seal Key'' and a ``Provisioning Key'' are burned into the die of an SGX-enabled processor.
The provisioning secret is generated by Intel at the key generation facility and also stored by the provisioning service for later identification.
The seal key is generated by the processor and not known to Intel~\cite{sgx-explained}.

% nice overview: https://sgx101.gitbook.io/sgx101/sgx-bootstrap/enclave/interaction-between-pse-and-application-enclaves

Intel distinguishes local and remote attestation.
Both describe a process of an enclave proving its identity to a second dedicated enclave.
As a result, two enclaves on the same platform have established trust and can exchange information. 
During attestation a dedicated instruction (\emph{EREPORT}) defined by the SGX-SDK is used to create a report that cryptographically bundles,
most importantly, a measurement of the enclave (\emph{MRENCLAVE}),
a certificate (identity information) of the enclave's software (\emph{MRSIGNER}) and a hardware MAC to prove authenticity.
Other information such as the CPU's security version number is included but not further explained herein.
The attestation report can then be used to verify that it was produced by identified software isolated by genuine (Intel-) hardware.

Remote attestation is executed after the local attestation has been executed successfully and a local quoting enclave has established trust in the to-be-attested enclave.
Through remote attestation a third party (challenger) can remotely establish trust in an SGX-enclave and ensure the genuineness of the executed soft- and hardware.
Section~\ref{sec:attestation} explains attestation in more detail.


==> shepherd_version/02_background_sgx_frameworks.tex <==
% \subsection{SGX Frameworks}\label{sec:background:sgx_frameworks}

% \fg{
%     TODO: Point out spectrum of SGX framework approaches along the aspects of generalidity and security.
% }

% % How SGX systems integrate attestation and how this integration doesn't help against our assumed adversary

% \paragraph{SCONE}
% SCONE~\cite{arnautov2016scone} is a framework to execute unmodified applications in at Intel SGX \gls{tee}.
% The attestation protocol of SCONE has been described by Trach \etal{} for in Shieldbox~\cite{trach2018shieldbox}.
% In SCONE, the initial enclave is built from the program's binary together with the dynamic libraries as indicated by the binary' ELF.
% \footnote{The \gls{sgx} \gls{sigstruct} is loaded from the ELF as well.}
% When an enclave starts it connects to the SCONE \gls{cas}~\cite{palaemon}, via an TLS channel using mutual authentication.
% %Said certificate is randomly generated by the enclave after it started.
% The TLS channel is bound to the enclave's identity by sending an \gls{sgx} quote to the \gls{cas} where the enclave certificate is hashed into the \texttt{reportdata} field.
% \gls{cas} builds trust into the channel by verifying the quote and ensuring that the embedded certificate hash matches the incoming channels client certificate.
% \rk{report oracle has not been introduced}
% However, an adversary with access to a report oracle can pretend that the channel terminates in the enclave.
% They generate the certificate and establish the TLS connection from outside an enclave and use the report oracle to craft the \gls{sgx} quote necessary to trick the \gls{cas}.

% \paragraph{SGX-LKL}\label{sec:sgx-lkl}
% SGX-LKL~\cite{priebe2019sgx} implements a similar architectural approach but misses the verification and attestation service.
% \rk{Extend!}\dots{}
% From SGX-LKL's approach it becomes apparent that whatever the enclave puts into \texttt{reportdata} field, our assumed adversary is able to exploit.
 
% \paragraph{Graphene-SGX}
% Graphene-SGX~\cite{tsai2017graphene}, an open-source implementation for \gls{sgx} of the original Graphene library OS and similar to Haven~\cite{baumann2015shielding}, runs a complete library OS inside of SGX enclaves.
% Graphene-SGX mainly relies on a \texttt{manifest} file to protected applications by statically listing all files accessed during the runtime of enclave.
% The manifest also contains user defined security policies. 
% Hence, the manifest allows for a fine granular but static definition of trusted resources.
% \rk{Write about attestation?}



==> shepherd_version/02_background_threat_model.tex <==
\vspace{-2mm}\subsection{System \& Threat Model}\label{sec:threat_model}

All systems building upon \gls{sgx} must rely on its hardware-assisted attestation mechanism to establish trust.
In \gls{sgx}' threat model the processor is the only trusted component.
In this section, we assume an attacker who is not able to violate the security guarantees of \gls{sgx}.
%However, they can exploit the user's enclave to create attestation reports with arbitrary \texttt{reportdata} content.
\textcolor{blue}{However, they can create enclaves in the same environment as the user to impersonate the user's enclave and create attestation reports with arbitrary \texttt{reportdata} content}.
%\footnote{The interested reader may note that most \gls{sgx} systems specifically state that they cannot protect software that contains remotely exploitable bugs.
%Such reader will be surprised by our findings in Section~\ref{sec:report_oracle} were we show attack scenarios that require no such exploitation.}
%Here we focus on the additional security capabilities contributed by the integration.

Our system model has the following assumptions:
\begin{itemize}
    \item The software is developed and distributed by a trusted software developer.
    \item A trusted signer prepares the software for execution inside of \gls{sgx}. This is done with the help of a trusted \gls{sgx} framework that enables the execution of legacy software inside of \gls{sgx}. In particular, the signer creates a valid \gls{sigstruct}. 
    \item The user customizes the \gls{sgx}-enabled software by configuring it. The configuration (files, environment variables, program arguments, etc) is secured through trusted means provided by the \gls{sgx} framework.
    \item Developer, signer and user and their systems are benign and have means to exchange information about the integrity of the software securely.
    \item The customized software is transmitted and executed in an \gls{sgx}-enabled environment under control of the adversary.
    \item The utilized \gls{sgx}-environment delivers its security goals. For example, the remote attestation mechanism and infrastructure are trusted and we assume \gls{sgx} processor implementation is not exploitable.
    \item The attestation protocols are known to the adversary, \ie{}, no security through obstruction.
\end{itemize}
%\vspace{-1mm}
Note that the developer, signer and/or user roles might be shared by the same entity.
SGX cannot protect secrets at rest for previously unknown platforms.
Therefore, secrets can not be part of an enclave, but must be provisioned after the enclave has been found trustworthy via remote attestation.

In our system model the user wants to run a native application in an enclave in a public cloud.
The enclave needs a configuration to run and secrets to, \eg{}, authenticate to other services or decrypt sealed file system content.
The user utilizes \gls{sgx} remote attestation to build trust into the remote enclave before sending its configuration via a secure channel.
The secure channel is bound to the enclave via attestation.
The attestation and configuration tasks are delegated to a trusted verifier service on behalf of the user.

Note that our system model is closely modeled after what we see in existing systems:
For example, SGX-LKL 
%\footnote{We refer to the ``legacy'' branch of SGX-LKL, which is also described in the ATC paper, as the `oe-port' branch did not support remote attestation at the point of writing.}
enclaves load an encrypted disk image and set program arguments and environment variables according to the configuration~\cite{priebe2019sgx}.
The trusted verifier service is the \texttt{sgx-lkl-ctl} command line tool that attests the enclave and delivers the configuration.
The secure channel is based on wireguard and it is bound to the enclave by adding the enclave's public wireguard key in its reportdata field.
In a SCONE, program arguments, environment variables, and session secrets are retrieved from the configuration and encrypted file system content is opened before the internal program is loaded.
The SCONE \gls{cas}~\cite{palaemon} is the trusted verifier service to which the enclave connects and from which it retrieves its configuration through encrypted channel.
% where the enclave's private key is hashed into the reportdata field.
Recently, remote attestation was added to Graphene-SGX~\cite{tsai2017graphene} as a shared library that uses RA-TLS as secure channel bound to the enclave.
 % Must investigate %


==> shepherd_version/03_attack.tex <==
\vspace{-2mm}\section{Remote Attestation Bypass Attack}\label{sec:attack}


% \begin{table}[h]\footnotesize
%     \begin{tabular}{ >{\arraybackslash}p{0.24\columnwidth} >{\centering\arraybackslash}p{0.2\columnwidth} >{\centering\arraybackslash}p{0.17\columnwidth} >{\centering\arraybackslash}p{0.2\columnwidth} }
%         \rowcolor{gray!15}
%          & SGX-LKL & SCONE & Graphene    \\
%         Framework & \(\bullet{}\) & \(\bullet{}\) & \(\bullet{}\) \\

%         \multirow{2}{0.24\columnwidth}{Program \& Libraries} & \multirow{2}{0.2\columnwidth}{\centering{}\(\circ{}\)} & \multirow{2}{0.17\columnwidth}{\centering{}\(\bullet{}\)} & \multirow{2}{0.2\columnwidth}{\centering{}\(\bullet{}\)} \\ \\
        
%         File System State & \(\circ{}\) & \(\circ{}\) & \(\bullet{}\) \\
        
%         Verifier Identity & \(\circ{}\)  & \(\circ{}\) & \(\circ{}\) \\
%     \end{tabular}
%     \caption{Data hashed into the enclave measurement value}
%     \rk{Integrate table as text}
% \end{table}


% In this section, we describe the remote attestation bypass attack in which the adversary uses an enclave trusted by the user to gain the user's secrets.
% First we provide an overview about remote attestation in \glspl{tee}, then we show the vulnerability of the general remote attestation protocol provided in \glspl{tee}.
% Afterwards, we describe the attack against remote attestation in Intel \gls{sgx}. 

This section explains how an adversary can exploit the remote attestation bypass attack using an enclave trusted by the user to access their confidential information.
We provide an overview of remote attestation in \glspl{tee}, show the vulnerability in the protocol, and describe the attack in Intel \gls{sgx}.


\vspace{-2mm}\subsection{Attestation Overview}\label{sec:attestation}

\begin{figure}[t!]
	\centering
    \vspace{4pt}
	\includegraphics[scale=0.45]{figures/remote-attestation-overview}
	\caption{General remote attestation protocol in \glspl{tee}.}\label{fig:remote-attestation-overview}
        \vspace{-6mm}
	\Description{No description.}
\end{figure}


%\rk{
%Note that the hardware resident identity information of the enclave (\ie{}, MRENCLAVE, MRSIGNER, and enclave attributes) cannot be forged.
%Intel SGX defines that the report additionally contains data that identifies the quoting enclave.
%This in turn defines that only the quoting enclave can validate the given report.
%For remote attestation, an enclave first executes the local attestation for the Quoting Enclave.
%The Quoting Enclave then validates the local-attestation report and signs it using the EPID key.
%The challenger can then use the signed report, called quote, to establish trust in the enclave by verifying the validity of the quote.
%}

%Introduced by the Trusted Computing Group for Trusted Platform Modules (TPM)~\cite{tpm} (remote) attestation
Remote attestation allows a verifier to assert a certain state of an application is running in a \gls{tee} (see Figure~\ref{fig:remote-attestation-overview}).
On the device, there is a prover entity (\emph{Quoting Enclave} in \gls{sgx}) able to produce the evidence for the state of the application before running it; and securely send it to the verifier.
The attestation process consists of two major parts: \emph{(i)} Characterization of the application's current state (the measurement process to create the evidence, called \emph{quote} in \gls{sgx}); and \emph{(ii)} Secure transfer of the evidence to the verifier.

%We distinguish remote and local attestation.
%In local attestation, the verifier has direct access to the prover and trusts it implicitly because they share the same \gls{tcb} (the same processor in case of \gls{sgx}).
%If the verifier doesn't trust the prover a priori, it must establish said trust before it can rely on the evidence.
%This is necessary for remote attestation where verifier and prover run on different machines.
%The trustworthiness of a prover can be establish with trust database knowing all trustworthy prover \glspl{tee} to which the \gls{tee} offers access to via an API (attestation service).
The measurement is used to prove the application is running in a correct state (\eg{}, correct code) inside enclaves of \glspl{tee}.
It can be a cryptographic hash over the binary of an application (see \S{}\ref{sec:background}) or could also contain other target information for the attestation.
The measurement is then signed using a hardware-protected certified key unique to the device to create the evidence or quote that can be verified by the verifier. 
%protected in the \gls{tcb} of the \gls{tee}, \eg{}, the CPU hardware,
The certified key ensures the \emph{authenticity} of the remote attestation protocol.
To ensure the \emph{freshness} of the evidence, the verifier includes a \emph{nonce} into the challenge in its request to the remote enclave.

Figure~\ref{fig:remote-attestation-overview} summarizes the general remote attestation workflow in \glspl{tee}.
Before launching an application in an enclave deployed on the remote device/host, the measurement process creates the attestation evidence.
When the verifier wants to verify if the remote application has an expected state, it sends a request with a nonce to the remote enclave (step (1)).
The enclave combines the nonce with the measurement, signs it to create a report using attestation keys (stored in CPU hardware), and sends it to the prover (step (2)).
The prover verifies the report, signs it to create the evidence (\ie{}, quote), and sends it back to the verifier (step (3) and (4)).
The verifier checks the signature and certificate with the help of the trusted third-party, \eg{}, the attestation service of the \gls{tee} provider,
and checks that the measurement indicates the start of the expected enclave (steps (5) and (6)).
Note that in other TEEs, e.g., AMD SEV SNP, the enclave is a secure virtual machine (VM) and the remote attestation and quoting are performed by the AMD Secure (Co-)Processor.

\input{03_attack_overview.tex}

\vspace{-2mm}\subsection{Attack Examples}\label{subsec:sgx-attack}
In this section, we show the practicability of the previously described attack by describing our attack against state-of-the-art \gls{sgx} frameworks.
Compared to previous work~\cite{van2020sgaxe}, our approach does not attack the sealing mechanism of \glspl{tee}.
We show our attack against applications running in SCONE as well as in SGX-LKL which support transparent remote attestation for users.

\vspace{-2mm}\subsubsection{Attacking Python and NodeJS in SCONE}
%In this section we show how we exploited applications protected by SCONE.
%We describe how we built the necessary components for the attack and walk through the process of the attack itself.
%The description focuses on Python since the attack on NodeJS only differs in a single aspect that we will point out where appropriate.

We assume the Python application's files are protected with SCO\-NE's file system encryption.
The application's configuration, including the Python interpreter's expected enclave measurement and signer identity and the file system encryption key, are stored in SCONE's \gls{cas}~\cite{palaemon} the secrets management service (running in an enclave itself).
SCONE enclaves connect to \gls{cas} during startup to obtain their configurations and transparently provide them to the executed application.
For this, \gls{cas} ensures that the enclaves match the user-provided expectations, utilizing \gls{sgx} attestation.
That is, in SCONE, \gls{cas} functions as the attestation verifier.

\vspace{-2mm}\subsubsection*{TEE Impersonator}
For building a \gls{tee} impersonator for SCONE we adapted the existing CAS-client implementation.
The \gls{sgx} report retrieval mechanism of the client is configurable through a callback mechanism.
Hence, we only needed to implement a client for the SCONE report server implementation (discussed below) and configure the CAS client to use it.
Together with the necessary argument parsing the \gls{tee} impersonator implementation consists only of \(75\) lines of code.

\vspace{-2mm}\subsubsection*{Report Server}
In SCONE, a program's file system is not reflected in the enclave measurement value.
Any Python program utilizing the same Python interpreter in SCONE uses an identical enclave and can not be distinguished by the verifier.
The verification of the actual Python (byte-) code that is stored in the encrypted file system is delegated to the runtime.
With the configuration, the runtime obtains the expected state of the file system and uses this information to ensure files have not been tampered with during execution.
This delegation is precisely the exploitable culprit as the passed configuration is not verifiable through attestation.
%And, if not configured as expected by the user, the runtime will not enforce the expected file system state.
Based on this, an adversary can invoke the user's Python enclave and configure it to run a report server program instead of the user's application (after attestation).

For the attack, we implemented a \textit{report server} with a simple Python socket server that receives the information necessary to query the report, in particular the \texttt{reportdata}, via the network.
%The data is transferred without encoding or framing as plain bytes.
%Start and end of messages is known due to their constant size.
The \gls{sgx} report is obtained through a custom Python C module in which we use the \texttt{EREPORT} \gls{sgx} hardware instruction in assembly.
The resulting report is sent via the same network connection towards the \gls{tee} impersonator.
Our attack requires dynamic loading of code at runtime as required by the Python interpreter.
%, a configuration option that is represented in the enclave measurement and, thus, not manipulatable by the adversary.
%However, since Python itself requires dynamic loading the user needs it to be activated.
The entire report server implementation consists of \(33\) lines of Python code and \(76\) lines of C code.
For the attack on NodeJS, we implemented a separate \textit{report server} as the interpreter binaries.
%It offers the exact same interface as the Python server such that we have a generic \gls{tee} impersonator.
NodeJS allows the execution of native (C) code through C++ addons that are loaded dynamically at runtime.
We implemented the server loop in \(22\) lines of JavaScript and the addons executing \texttt{EREPORT} required \(67\) lines of C++ code.

\vspace{-2mm}\subsubsection*{Attack Procedure}
%The adversary can mount independently from the user since SCONE CAS is a service.
For the attack, the adversary first starts the \textit{report server} built from the enclave trusted by the user.
%Note that, according to our threat model, the adversary is able to start the user's enclave without any restrictions.
Then the adversary invokes the \gls{tee} impersonator configuring it with the user's configuration id as well as the addresses of the necessary services and waits for the \gls{tee} impersonator to yield the user's configuration.

The \gls{tee} impersonator connects to \gls{cas} and requests the user enclave's configuration.
The connection is established via a secure TLS channel whose certificate key's are used to ensure authenticity of the connection, \ie{}, ensuring the channel's integrity but also that the channel is terminated in the expected enclave.
In response \gls{cas} will demand a suitable remote attestation quote (SCONE, EPID, or DCAP quotes are supported).
Depending on the system capabilities an appropriate mechanism is chosen by the impersonator and the necessary \gls{sgx} report is queried from the report server.
The report server is instructed to incorporate the \gls{tee} impersonator's certificate key into the report's \texttt{reportdata} field undermining the channel's authenticity.
The verifier (\gls{cas}) is unable to detect the manipulation because the quote is valid, it shows the expected enclave is running and the TLS channel utilizes the expected certificate whose key is incorporated into the report.
Thus, it grants access and delivers the requested configuration.

\vspace{-2mm}\subsubsection{Attacking Python in SGX-LKL}\label{sec:attack_lkl}
%In this section we show our attack against SGX-LKL.
%Similar to above, we first describe the necessary components and how we built them and then explain the process of the attack.
%We will focus on Python again, but as we will show this attack is effective against any program running in SGX-LKL.

In SGX-LKL, the enclave starts a simple attestation and configuration service when invoked with \texttt{sgx-lkl-run}.
The user then connects to that service using the \texttt{sgx-lkl-ctl} tool and attests the enclave.
For this, the tool shows the \gls{sgx} report/quote details on the screen.
After verification of the shown details, the user invokes \texttt{sgx-lkl-ctl} again to transmit the enclave configuration, which contains the disk encryption key.
SGX-LKL uses encrypted disk images to load code into the enclave.
Having received the configuration, the enclave runtime accesses the disk and invokes the user application.

SGX-LKL implements additional restrictions to ensure the integrity of the attestation procedure.
For example, the runtime enforces that attestation and configuration is only done once.
Integrity of the attestation and configuration procedure is enforced by a public wireguard key that is provided to the enclave during invocation.
That is, the enclave will only interact with attestation and configuration requests originating from the benign user.
Furthermore, we assume the system is configured to run in release mode, which adds additional restrictions enforced by SGX-LKL:
The disk image (program) must be encrypted and the SGX-LKL will not start the user program without attestation.
We will show beneath that only this last restriction influences the attack but does not mitigate it.

\vspace{-2mm}\subsubsection*{TEE Impersonator}
SGX-LKL's attestation and configuration interface is implemented in C and uses \emph{protobuf} for message framing.
We implemented the SGX-LKL impersonator in Python.
It opens the attestation and configuration ports and waits for the user to connect.
%Connections handled by the impersonator are in clear-text.
SGX-LKL utilizes Wireguard (VPN) to establish secure channels.
We instruct the host \gls{os} to provide the VPN expected by the client instead of handling these details in the impersonator.
Upon start, the impersonator is configured with the nonce expected by the user and the public wireguard key the adversary configured the VPN with.
Our implementation consists of \(236\) lines of code and  \(\sim\)\(2000\) lines of generated \emph{protobuf} Python code.

\vspace{-2mm}\subsubsection*{Report Server}
The fact that SGX-LKL uses encrypted disk images and that the enclave is attested before the user code can be loaded -- since being encrypted -- hints that attestation in SGX-LKL ensures the integrity of the framework but not the user application.
User application integrity verification is implemented by the runtime by verifying the disk image's integrity.
In consequence, two different programs running in SGX-LKL will, from \gls{sgx} attestation perspective, be the same as long as they use the same version of SGX-LKL.
Consequently, the verifier can not distinguish them posing little restrictions for our report server implementation.
%Therefore, there are little restrictions for the report server's implementation.
We implemented it in \(152\) lines of C code.
%with a protobuf RPC interface for the impersonator to connect to and request the necessary \gls{sgx} report.

\vspace{-2.5mm}\subsubsection*{Attack Procedure}
The attack on SGX-LKL requires the adversary to interfere with the commands sent by the user.
%However, note that, this is rather a complication.
The adversary is in control over the machine on which the user wants to execute the enclave which allows them to execute all necessary actions.
Before the actual attack the adversary prepares an encrypted disk image containing the report server.
When the user attempts to start their enclave with \texttt{sgx-lkl-run},
she provides their public wireguard key and a nonce (and the desired disk image) to the command to ensure the enclave can only be controlled by them.
%At this point it is clear which version of SGX-LKL the user expects.
The invocation command is intercepted by the adversary and they start the report server's disk image, however, with the adversaries public wireguard key using the \texttt{sgx-lkl-run} command.
This enclave is then attested and configured by the adversary to execute the report server.
At the same time the adversary starts the SGX-LKL impersonator and configures it to put a public wireguard key controlled by the adversary into the \gls{sgx} report.
Incoming requests to the user's enclave are forwarded the configuration interface of the SGX-LKL impersonator using the same wireguard guard key.
Afterward, the adversary waits for the attestation request from the user that is forwarded to the SGX-LKL impersonator.
It queries the report server for the necessary \gls{sgx} report containing the adversary's wireguard key in the \texttt{reportdata} field.
The report is sent back to the user for inspection.
At this point the user has no chance to detect the manipulation, seeing only a valid \gls{sgx} report for the expected SGX-LKL enclave.
Thus, they decide to trust it and use the embedded wireguard key to establish a secure connection to send the configuration over.
The wireguard key is embedded in the report
% though, is under the control of the adversary and,
and the connection is established with the wireguard setup in the malicious host \gls{os} responded to by the impersonator, revealing the configuration to the adversary.

% Note that, none of the additional restrictions implemented by SGX-LKL could prevent the attack.
% Only the requirement to use an encrypted disk in release mode is reflected in the enclave measurement in SGX-LKL.
% Thus, the adversary had to use an encrypted disk image for their report server and configure it through attestation.
% The requirement that the attestation and configuration must originate from the user, was not reflected in the measurement and could be therefore ignored.

%In summary, in this section we have explained the remote attestation bypass attack and shown how it exploits existing state-of-the-art \gls{sgx} frameworks.
%Further, we demonstrated that existing mitigation strategies in SGX-LKL framework are insufficient.


==> shepherd_version/03_attack_overview.tex <==
\vspace{-2mm}\subsection{Remote Attestation Bypass Attack Overview}\label{sec:attack_overview}

\begin{figure}[t!]
	\centering
	\includegraphics[scale=0.44]{figures/remote-attestation-attack-overview}
    %\vspace{2mm}
	\Description{Overview of remote attestation attack: If the application dynamically loads libraries and its configuration during runtime, an attacker can load compromised libraries or manipulate the configuration of enclaves.}
	\caption{The overview of remote attestation attack.}\label{fig:remote-attestation-attack-overview}
        \vspace{-4.5mm}
\end{figure}

A major security issue in remote attestation of current TEEs is that the measurement process is only conducted before running the application and it cannot be performed during runtime.
If the application dynamically loads libraries and its configuration during runtime, an attacker may load compromised libraries or manipulated configurations into enclaves (see Figure~\ref{fig:remote-attestation-attack-overview}).
The attacker can create a genuine evidence (quote) using the malicious enclave since it has correct measurement and send this evidence to the verifier to bypass the remote attestation (steps (2), (3), and (4)).
The attacker can further steel secrets of applications after bypassing the remote attestation (details in \S{}\ref{subsec:sgx-attack}).
Applications with the pre-compiled binaries are vulnerable to this attack since their behavior is mainly determined by their configuration.

For this work we imagine a user who wants to run their legacy application in a potentially adversarial cloud environment.
The user protects the application's code and data during runtime using an \gls{sgx} framework.
At runtime application's behavior significantly depends on data the application consumes (mainly from the file system), \eg{}, configuration files or mounted volumes.
Remote attestation is subsequently used to establish that the application has not been modified by an adversary prior to execution.

The adversary needs two components for the attack: an \textit{TEE impersonator} and a \textit{report server}.
The \gls{tee} impersonator implements the attestation protocol utilized by the verifier, while the report server generates \gls{sgx} reports with arbitrary, adversary-chosen \texttt{reportdata} fields.
Note that the \textit{TEE impersonator} is not required to be executed inside of an enclave.
The \textit{report server}, on the other hand, must be executed inside of an enclave, fulfilling expectations by the verifier and allowing it to generate \gls{sgx} reports.
Next, we describe how the adversary can build a \textit{report server} from an enclave without this being reflected in the enclave's measurement.
%Once we discussed some concepts we apply them to SCONE and SGX-LKL.

\vspace{-2mm}\subsubsection{Creating a Report Server}\label{sec:report_oracle}

A report server is an enclave that produces \gls{sgx} reports with arbitrary report data upon the adversary's instruction.
The concrete steps and complexity of creating a report server from an arbitrary enclave vary but three operations must be implemented:

\begin{itemize}
    \item The desired report data and target information must be copied into enclave memory.
    \item The \gls{sgx} report generation must be invocable.
    \item The created report must be delivered to a verifier.
\end{itemize}

%For this discussion we assume that any enclave has some form of receiving and sending data from the outside world.
Network connections, file system interfaces, the terminal, or reading of environment variables can be utilized for communication.
%Even encrypted file systems can be used, if the adversary is able to configure the encryption key.
Arguably any enclave must provide some form of input and output to do useful work.
We also assume that any enclave of interest would allow for \gls{sgx} report generation given that \gls{sgx} attestation is to be used to securely provision configurations to the enclave and that remote attestation can be used throughout the lifetime of an enclave.
For example, attestation is used to convince users of a service of the enclave's trustworthiness or sign data produced by the enclave.
Many \gls{sgx} frameworks voluntarily expose attestation features including setting arbitrary \texttt{reportdata}:
SCONE~\cite{arnautov2016scone} exposes report generation via C functions to user code.
Occlum~\cite{shen2020occlum} provides special \texttt{ioctl} system calls.
Gramine~\cite{Gramine} (initially Graphene-SGX~\cite{tsai2017graphene}) exposes the report generation via pseudo-files in \texttt{/dev/attestation}.
Hence, we assume that the three necessary operations are present in any enclave an adversary would be interested in.

With these building blocks available, the adversary needs to gain control over the enclave such that it uses these operations according to the adversary's desire.
Typically, such control is obtained by exploiting vulnerabilities in the enclave's code and, thus, many frameworks use memory-safe languages to mitigate such risks.
However, we found a significantly simpler approach: through configuration.

% \subsubsection*{Vulnerability Exploitation and Return Oriented Programming}
% \fg{
%     Pick up the reader who thinks controlling a trusted enclave from somebody else is complicated.
% }
% \fg{
%     first obvious ``solution'', often discussed already -- well known
%     sgx already got lost of critic for this attack vector and the common response is that if the application is vulnerable there is nothing to win here or the usage of \gls{sfi} techniques that
%     prevent a vulnerability from being exploited.
%     Also \gls{cet}, \ie{}, shadow stacks and indirect branch tracking, that is available on new processors prevents return oriented programming.
% }

\subsubsection*{Creating a Report Server by Configuration}
%Our threat model allows adversaries to use significantly wider attack vectors than in a more traditional model.
%In particular, they can start and configure the user's enclave arbitrarily often.
Our threat model allows adversaries to start and configure the user's enclave arbitrarily often.
They can also run their own verification and configuration component that delivers the desired configuration to the enclave.
In summary, if not prohibited by the enclave itself, the adversary can run the user enclave with an arbitrary configuration.
% For example, they could enable flawed features or plugins of the software that would ease their \gls{rop} attempts.
% However, we have found that this is not necessary in many cases.
% Often the \gls{sgx} framework or the user application are configurable to a sufficient extend.
% We want to highlight three strategies with which the adversary can create a Report Server through carefully configuring a trusted enclave.
%

If the software's configuration that is not reflected in the enclave measurement (\S{}~\ref{subsec:sgx-attack}) dictates the to-be-loaded program, the adversary can simply start a report server implementation.
In other cases, the user application might be substantially configurable.
This is mostly always the case for language interpreters, for languages such as Java, Python, JavaScript, Ruby, etc.
In some frameworks, these interpreters are already the entire enclave while the actual program is loaded from the file system at runtime.
For example, when Java applications, such as Wildfly/JBoss or Tomcat, are executed the exact same interpreter and, thus, enclave is used.
Thus, the adversary can configure the interpreter enclave to load their report server implementation in the necessary language, for example, Java without the attestation report reflecting this.

Alternatively, any program that loads dynamic code during runtime can be used by the adversary.
Dynamic loading is broadly used to load optional features into a program.
For example, Apache \texttt{httpd} loads only the configured modules, or NGINX's dynamic module extends its features using dynamically loaded code.
%Even \texttt{sudo}, a popular tool to gain root privileges, utilized dynamically loaded code for name resolution\footnote{A recent exploit for \texttt{sudo} using dynamic code for exploitation: \url{https://www.qualys.com/2021/01/26/cve-2021-3156/baron-samedit-heap-based-overflow-sudo.txt}}.
Since the dynamic code is only loaded during runtime, it is typically not reflected in the enclave measurement and, thus, manipulating it isn't revealed through attestation.
Therefore, the adversary can patch existing functions such that they execute the desired operations.
%For example, NGINX could be extended with an additional compression methods via its dynamic modules mechanism.
%For example, the adversary could modify the module's file, such that every time the web server calls into the module additional code is executed.
This code could read the desired \texttt{reportdata} from a file, query the \gls{sgx} report and write it into another file implementing a report server.
With this, the adversary could trigger the code by querying a site with the appropriate compression algorithm requested.

\textcolor{blue}{A straightforward way to handle the attacks is using static linking for applications. However, it also comes with the cost of increased binary size which makes booting time slow, compatibility issues, performance overhead, and resource redundancy. For interpreter languages, e.g., Python they need to pack dependencies with interpreter engines which is cumbersome. It requires heavy engineering, especially with complex libraries such as TensorFlow. }

\textcolor{blue}{Besides SGX, other TEEs, such as AMD SEV and Intel TDX, have a similar issue since these TEEs only perform measurements and ensure the integrity of confidential VMs after the booting process. During computation, these TEEs do not perform any measurements if shared data or libraries from the host are loaded to the VMs; it requires carefully checking or adding their measurement during the boot process. If there is no shared data or libraries between VMs or with the host, an attacker can just boot the VM from a victim and perform, e.g., side-channel attacks on the VM in a lab environment.}



%As mitigation some frameworks, \eg{}, SCONE, prevent dynamic loading by default and reflect this also in their enclave measurement.
%Dynamic loading typically is required by users applications and, thus, allowed the SGX frameworks (\eg{} SGX-LKL) are exploitable as we will show in the following.



==> shepherd_version/04_protection.tex <==
\vspace{-2.5mm}\section{Attestation Protection Mechanism}\label{sec:protection}

%\rk{We need a architecture/protection figure of the improved remote attestation (our contribution) here.} -> we don't have space for it

The remote attestation bypass attack uses fundamental technical properties built into \gls{sgx} rendering a verifier unable to distinguish between a newly started enclave without a configuration and an enclave pre-configured by an adversary.
In the following, we detail our protection mechanism against the remote attestation bypass attack.

% There are fundamental technical properties built into \gls{sgx} that are exploited by the attack.
% That is \gls{sgx} enclaves can attest themselves arbitrarily often, however, the trustworthy data obtained by the verifier is static, it doesn't change throughout the enclave's life.
% Therefore, the verifier is unable to determine whether an enclave requesting a configuration is a newly started and not configured or whether it was configured before by the adversary.

\vspace{-2mm}\subsection{Design Space}\label{subse:protection-requirements}

Different approaches for protection mechanisms are possible due to the complex design space of remote attestation and the software stack involved.
However, we adhere to two common characteristics of modern cloud-native applications:
An enclave's configuration might not be known beforehand, \ie{}, program arguments of spawned sub-processes might be computed dynamically by the parent process and files can be used to transfer data in between processes.
Hence, the protection must be \emph{flexible} to adapt to the dynamic behavior of applications. 
and the protection mechanism must be practical, \ie{}, usable with existing hardware.
%For starters, hardware development cycles take sorely long.
%Further, existing machines would be left vulnerable, which may not only lead to a loss of financial investment but also waist environmental resources unnecessarily.
%Lastly, from a systems development point of view, we believe that composable software components of the shelf are a great driver of efficiency and innovation.
%With regards to \gls{sgx} this means that an enclave's \gls{sigstruct} should be created by the individual software developers and not the integrator.

\vspace{-1mm}\subsection{General Solution Principle}

We prevent the shown exploitation by enabling the verifier to establish that an enclave is fresh and complete, \ie{}, it cannot have received a malicious configuration beforehand.
One possibility to prevent the attack would be to forestall the adversary configuring the enclave into a report server.
However, preventing the adversary from freely configuring the enclave would also contradict our \emph{flexibility} requirement.
Next, we discuss solutions with specific shortcomings before presenting our solution -- \emph{Singleton Enclaves} (\S{}\ref{sec:sin-enclave}).

\vspace{-2mm}
\subsection{Naive Approaches}

%\fg{Naive Approaches are insufficient - convince the reader this is a complicated problem and simple solutions are flawed. Also show how we ended up with our solution.}

% \subsubsection*{Comprehensive Enclave Measurement}

% %This is to remind them that Graphene's and Occulums approach is insufficient.
% In a framework with (fully) comprehensive enclave measurement, the enclave measurement determines all data and configuration the enclave will ever access throughout its life.
% That is, the enclave's entire behavior is determined by the enclave measurement.
% Note that this also includes input data.
% This must be secure as previously pointed out in Section~\ref{sec:background:sgx_frameworks}.
% However, this approach severely limits the usability of the enclave.
% To reemphasize, all configuration and input data is part of the enclave measurement.

% This approach conflicts with our requirements in two points.
% First, any configuration or data change requires the user to sign the new enclave measurement - a burden we don't want to put on the user.
% Secondly, dynamic spawning of child processes or data exchange between processes is not possible.
% Therefore, we deem it unsuitable.

%\vspace{-2mm}
% \subsubsection*{Restricted Runtime Operations}
\myparagraph{Restricted Runtime Operations}
%Only execute if attested.
A naive approach implemented in SGX-LKL allows the enclave to run only if it is attested and its configuration is provisioned via a secure channel that must be terminated by the verifier.
%That is the enclave will only accept configurations from the trusted verifier.
Still, we are able to exploit it (as shown before) because the trusted verifier must also be configured in the enclave and this configuration is not reflected in the attestation report and, thus, can not be verified.
% by the verifier with remote attestation.
Therefore, the adversary can start an enclave, configure it to trust the adversary and start a report server.
This report server can then be used to fool the user by pretending to be a fresh SGX-LKL enclave since its \gls{sgx} report neither reflects that it was configured already nor that its actually SGX-LKL runtime was configured to trust the adversary.

%\vspace{-2mm}
\subsubsection*{Using SigStruct}

As an alternative to the previous approach, the \gls{sgx} \gls{sigstruct} data structure could store additional information without the need for adaption of the software.
% as parts of the \gls{sigstruct} are directly visible to the verifier during attestation.
However, there are only very limited fields/space that can be freely controlled -- a couple of bytes.
Unfortunately, this is not enough to store a cryptographic identity but merely a config identifier. 
Using config identifiers is insufficient as their enforcement would have to be implemented in the verifier that is suspectable to manipulation by the adversary.
Imagine a \gls{sigstruct} stating that the enclave only accepts configurations with id A.
The adversary could simply accept that \gls{sigstruct} and ignore the restriction.
Alternatively, a hash of an entire config would be equivalent to the comprehensive enclave measurement solution but unfortunately would be too large for the data structure.

The \emph{MRSIGNER} field could also be used for the protection:
The enclave could only accept configuration that comes from a specific signer identity.
This approach would work, however, it requires the users to sign all individual enclaves themselves. %- no components of the shelf\dots.
We regard this approach as impractical for cloud-native applications.

\fg{We could improve the argument by saying that a singleton enclave reduces the attack surface -- There is a python that only accepts configurations from B, but one python program has a bug and enables the adversary to build a report oracle -- no python program of B is secure any more.
The \gls{sigstruct} offers fields that allow custom values that are signed by the signer key.
%~\footnote{Intel whitelisted signer keys are necessary to run enclaves in secure production mode on systems without \gls{flc}.}
One can use these fields to implement singleton enclaves based on the \gls{sigstruct} information or even use unique signer keys.
}
%\rk{Something is missing in the next line.}
%Also the signer key can, in principle~\footnote{Intel whitelisted signer keys are necessary to run enclaves in secure production mode on systems without \gls{flc}.}
%Therefore, this is only a viable solution if \gls{flc} is available., chosen arbitrarily.
%\rk{If FLC is available or if not?}

%\vspace{-2mm}
\subsubsection*{Using reportdata to show state}

As an alternative solution, one could include a config identifier or similar that proves the enclave was not configured already into the report data field of the report.
After all, the report must be created from the code that was measured in it, and thus, only that code could say it has not been configured at runtime.
SCONE and SGX-LKL have supported this approach, but using the report data field for such purposes is not secure in our threat model.
After an adversary manages to create a report oracle, she also controls the report data.
Consequentially, only fields the hardware sets can be trusted against a powerful adversary.

%\vspace{-2mm}
\subsection{Singleton Enclaves}\label{sec:sin-enclave}
\begin{figure}[!t]
    %\vspace{3pt} % vertically align the top of the figure with the fig in the left column 
    \centering
    \includegraphics[height=.25\textwidth]{figures/enclave-memory-layout.pdf}
    \caption{Enclave Memory Layout in \sys{}}\label{fig:solution:enclave_memory_layout}
    \vspace{-2mm}
    \Description{The Figure shows three memory layouts for enclaves. It is presented how \sys{} adds a single page to the enclave memory.}
    %\vspace{-1em}
\end{figure}

Our proposed protection mechanism is based on the following observations.
The attestation token is a mechanism that individualizes an enclave's measurement value (\texttt{MRENCLAVE}) in a verifiable manner such that re-attestation can be detected. This individualization happens at enclave construction time and is thus compatible with the binary distribution of software.

The basic idea behind our solution is that system software adds an additional page, the \emph{instance page} (see Figure~\ref{fig:solution:enclave_memory_layout}), to the enclave dynamically during enclave construction.
This page, in particular, contains an attestation token, and the verifier's cryptographic identity.
The attestation token is unique and generated by the verifier in a previous step.

Once the enclave is started it directly engages in attestation to obtain its configuration from the verifier.
In the request, the enclave sends its \gls{sgx} quote and the attestation token to the verifier via a secure channel.
The verifier calculates the expected \texttt{MRENCLAVE} based on the expected enclave, the attestation token and its own cryptographic identity and can thus, despite individualization, verify the enclave's integrity.

The enclave utilizes the verifier identity that is part of the \emph{instance page} to ensure it only obtains configuration for the intended verifier.
This prevents an adversary from supplying its malicious configuration and the verifier can utilize the attestation token to keep track of attested enclaves ensuring each enclave is attested exactly once.
In the following, we discuss the most important aspects of our approach.

%\vspace{-2mm}
\subsubsection*{Verifiable Enclave Extension}
Adding an additional page to the enclave must necessarily yield the desired different enclave measurement.
On the other hand, the verifier must be able to ensure the intended enclave was extended correctly, \ie{}, it was neither manipulated beforehand nor incorrectly extended.
Adding an additional page to the end of an enclave requires the additional execution of one \texttt{EADD} and four \texttt{EEXTEND} \gls{sgx} instructions.
From the perspective of the enclave measurement SHA-256 calculation, adding an additional page to an enclave constitutes four additional update calls.
This allows the verifier to pre-calculated the expected enclave measurement:
The SHA-256 calculation's internal state needs to be instantiated just before the initial (not yet individualized) enclave was finalized with \texttt{EINIT} and updated according with the expected content and position of the \emph{instance page}.
Position and content of the \textit{instance page}, as well as, the necessary SHA-256 calculation state can be computed by the verifier given the enclave.\rk{Do we explain how?}

\vspace{-2.5mm}\subsubsection*{On-Demand SigStruct Creation}\label{sec:sigstruct}

The \gls{sigstruct} is necessary to initialize an enclave (\S{}~\ref{sec:background:enclave_initialization}) but is only valid for a specific enclave measurement value (\texttt{MRENCLAVE}).
Since the attestation token individualizes the enclave's \texttt{MRENCLAVE}, a suitable \gls{sigstruct} must be computed for each individualized enclave before it can be initialized.
Computing the \gls{sigstruct} requires knowledge of the enclave signer's private key.
This key must stay private because: 
(a) If the adversary knows the key, we could only use the enclave measurement for verification.
(b) Any enclave with the signer identity A can derive signer identity A's \gls{sgx} sealing keys.
%If the adversary could sign his own enclaves, the \gls{sgx} sealing keys would be compromised.
(c) In SGX v1 only (signer) identities whitelisted by Intel can run enclaves in production mode. Compromised keys would be blacklisted.

In our protection mechanism, we distinguish \emph{singleton enclave} and \emph{common enclave}.
Both have the same base enclave hash -- the same software/code.
However, the singleton enclave must be attested and have a unique \emph{MRENCLAVE},
while the common enclave can be started arbitrarily many times.
The \emph{instance page} of the common enclave is zeroed such that the runtime can decide whether it requires attestation or not.

When querying the verifier for the attestation token, the common enclave's \gls{sigstruct} is also sent to the verifier.
The verifier ensures it matches the base enclave hash (if instantiated for the common enclave) and if so finalizes the base enclave hash according to the attestation token it just chose.
The verifier uses that value to create the (on-demand) \gls{sigstruct} for the particular singleton enclave he expects to be started according to the base enclave hash, the token and his certificate.
The \gls{sigstruct} is equivalent to the common enclave's \gls{sigstruct} except that the enclave measurement and the signature is exchanged.
That \gls{sigstruct} is sent to the starter who will initialize the enclave with the instance/singleton page and the received on-demand \gls{sigstruct}.
This ensures that the signer key never leaves the trusted verifier and only enclaves the signer previously signed already (he trusted) will be attested.
In consequence, our protection satisfies the requirements described in \S{}\ref{subse:protection-requirements}.
\textcolor{blue}{Note that the goal of the proposed protection mechanism is to allow users to create a singleton SGX enclave that can be extended to a singleton confidential VM. In the singleton confidential VM, the measurement process during booting time includes the user identity and security for that VM. In other words, an attacker cannot just boot a VM of the user since he/she cannot generate the unique measurement of the VM. Only after verifying that the VM is a unique single instance, secrets are injected into the VM.}

==> shepherd_version/05_evaluation.tex <==
%\vspace{-2mm}
\section{Evaluation}\label{sec:evaluation}

This section presents the experimental evaluation of \sys{} using micro- and macro-benchmarks.
%In the evaluation, 
We focus on the system behavior expected to be influenced by our contributions.
These are enclave signing, enclave construction and attestation.
During the signing \sys{}'s interruptible SHA-256 implementation is used.
We expect it to impose a lightweight overhead since it is implemented using only Rust, while state-of-the-art SHA-256 implementations use optimized assembly code and hardware acceleration~\cite{gulley2013intel}.
%\footnote{According to our system model, an enclave is signed only once. Thus, optimizing the enclave signing code was not our focus.}
An enclave based on \sys{} must query the verifier before the singleton enclave can be initialized.
This communication is necessary to get the attestation token and the on-demand \gls{sigstruct} and will slow down the overall application start.
Finally, the verification with \sys{} requires additional checks, which we expect to have only negligible influence.
After describing our evaluation settings (\S\ref{sec:eval:hardware-setup}), we discuss our results for the micro- (\S\ref{sec:eval:micro}) and macro-benchmarks (\S\ref{sec:eval:macro}).

\vspace{-2mm}\subsection{Experimental Setup}\label{sec:eval:hardware-setup}

We used a machine equipped with an Intel\textregistered{} Xeon\textregistered{} E-2288G CPU @ \(3.70\)\thinspace{}GHz ($8$ physical cores and activated hyper-threading) with SGX support and \(128\)\thinspace{}GiB of RAM.
The system uses a \(2\)\thinspace{}TB Intel\textregistered{} 660p M.2 using PCIe 3.0\(x\)4 as persistent storage.
The operating system is Ubuntu 18.04.5 LTS with Linux 4.15.0-142.
%and \gls{sgx} software support is made available through the \gls{sgx} OOT driver in the most recent version 2.11 built from source~\cite{driver}.
We compare \sys{}'s performance with the master version of SCONE v5.3.0 as baseline.
%with commit hash \fg{X}, which is a development version on top of SCONE v5.3.0. This version of SCONE uses Rust 1.47.0.
\sys{}'s implementation used the same version of SCONE.
%\sys{}'s implementation is built on top of the same version of SCONE.

\vspace{-2mm}\subsection{Micro-benchmarks}\label{sec:eval:micro}
%We provide a detailed analysis of the performance impacts of \sys{} with micro-benchmarks.
All micro-benchmarks have been executed with the Criterion benchmarking framework~\cite{criterion}.
The framework was configured to warm each benchmark for \(3\) seconds and afterwards perform measurements for at least \(120\) seconds taking \(20\) samples.
Variance is omitted as it was negligible throughout all benchmarks.
We report the mean runtime as reported by Criterion.

%The presentation of the micro-benchmarks is organized according to occurrence of the procedures when the system is used.

\vspace{-2mm}\subsubsection*{SHA-256 Computation Performance}\label{sec:eval:micro:sha256}

We investigate the overhead introduced by \sys{}'s interruptible SHA-256 implementation through evaluation of the hashing performance.
The benchmark hashes a buffer of various sizes and measures the throughput.
The buffer sizes correspond to differently sized \gls{sgx} enclaves, \ie{}, the size of an enclave program that must be hashed (measured) for attestation.

\begin{figure}[t]
    %\vspace{3pt} % vertically align the top of the figure with the fig in the left column 
    \centering
    \includesvg[width=.46\textwidth]{figures/evaluation/sha256MB.svg}
    \caption{SHA256 computation performance comparison.}\label{fig:eval:sha_comparison}
    %\caption{Calculation of a SHA256 checksum with different implementations.}\label{fig:eval:sha_comparison}
    \vspace{-2mm}
    \Description{A plot showing the evaluation of different implementations calculating a SHA256 checksum.}
\end{figure}

\input{05_evaluation_micro_plots.tex}

Figure~\ref{fig:eval:sha_comparison} shows a comparison of three SHA256 checksum calculations.
The baseline for this comparison is Ring v0.16.20~\cite{ring}, a crypto library for Rust that uses highly optimized code comparable to OpenSSL. %\footnote{A single run of \texttt{openssl speed sha256} reveals a speed of \(\sim 480\)\thinspace{}MB/s for a \(16\)\thinspace{}KB buffer.}.

\sys{}-BaseHash indicates the implementation of SHA-256 that produces a base enclave hash, \ie{}, the SHA-256 computation is interrupted before finalization of an enclave and the Base Enclave Hash is encoded instead of finalizing the SHA computation.
\sys{} indicates the variant of \sys{}'s SHA-256 implementation without interruptions, \ie{}, no base enclave hash is calculated but the SHA-256 computation is finalized directly.

The results show that SHA-256 implementation in the Ring library outperforms the interruptible variant of \sys{} for all buffer sizes.
Independent of the buffer size it yields about \(405\)\thinspace{}MB/s.
The \sys{} implementation, which is directly comparable to Ring, yields about \(180\)\thinspace{}MB/s.
This overhead is the result of \sys{} using less optimized code.
\sys{}-BaseHash basically shows an equivalent performance compared to \sys{} for sufficiently large buffer sizes.
For small buffers the overhead introduced by the additional encoding is significantly smaller than the effort necessary for SHA-256 finalization and, thus, \sys{}-BaseHash performs better with about 245~MB/s for 2~KB buffers.

Lastly, we measured the time it takes to finalize an enclave base hash into an enclave measurement.
This time is not influenced by the buffer size and requires constant \(32\)\thinspace{}\(\mu{}\)s.

\vspace{-2mm}\subsubsection*{Enclave Program Compilation}\label{sec:eval:micro:compilation}

In SCONE, during compilation, the enclave's \gls{sigstruct} is embedded into the binary's ELF.
The enclave measurement, which is part of the \gls{sigstruct}, is calculated by the SCONE signing tool using SHA-256.
For \sys{} we adapted the algorithm of SHA-256 to support interruption and to be able to measure individual enclave code based on a common base enclave (\S{}~\ref{sec:protection}).
We evaluate the overhead introduced by our changes by measuring how long it takes to compile a small C program that only contains a return statement in the main function.
We compare our results to compilation with the system C compiler (native) and SCONE (baseline).
%The available heap size of the produced enclave in baseline and \sys{} is varied to asses the influence of the enclave size.

As shown in Figure~\ref{fig:eval:compilation}, baseline and \sys{} introduce significant overhead.
% Compilation/native/32MB,heap,32993335.05824262,ns
% Compilation/baseline/32MB,heap,1520364471.7875,ns
% Compilation/singleton/32MB,heap,6257778456.75,ns
While native compilation takes only about \(0.033\)\thinspace{}s, baseline requires \(1.52\)\thinspace{}s and \sys{} \(6.26\)\thinspace{}s.
\sys{} needs about \(4\) times longer for compilation, while the ratio in the SHA-256 benchmark is just about \(2.25\).
Apart from the SHA-256 algorithm, there are no significant changes \sys{} introduces to the signer tool but
compared to the SHA-256 benchmark for which a continuous buffer is hashed at once, \ie{}, with a single call, the signer tool updates the SHA-256 computation iteratively.
Thus, we attribute this increased overhead to the less optimized code handling the entering and exiting of the hash computation.

\vspace{-2mm}\subsubsection*{SigStruct Signing and Verification}\label{sec:eval:micro:sig_struct_signing}

In \sys{} each enclave's measurement is unique and only known at execution time.
\gls{sgx}, on the other hand, requires a \gls{sigstruct} that is matching the enclave measurement.
Thus, in \sys{} individual \gls{sigstruct} must be created for each singleton enclave that is started, which is done by the verifier, \ie{}, SCONE \gls{cas} (\S{}\ref{sec:sigstruct}).
\gls{sgx} \glspl{sigstruct} are signed with an RSA key with \(3072\)\thinspace{}bits.
%RSA is known to be a computation expensive algorithm.
We assess the introduced overhead by measuring the time it takes to sign the \gls{sigstruct}.
During On-Demand \gls{sigstruct} generation, the verifier must assess the authenticity of received \glspl{sigstruct} to prevent tampering, therefore we also measure the time it takes to verify a \gls{sigstruct}.
As shown in Figure~\ref{fig:eval:sigstruct}, \gls{sigstruct} signing takes \(4.9\)\thinspace{}ms on average.
While verification takes \(0.4\)\thinspace{}ms on average (``Verify C.'' in Figure~\ref{fig:eval:sigstruct}).
We further measure the time the verification takes in case it fails ``Verify E.''. 
The results show no difference to correct verification.

\vspace{-2mm}\subsubsection*{Singleton Page Retrieval}

%In this experiment, we measure the entire overhead introduced by singleton page retrieval.
Next, we measure the entire overhead introduced by singleton page retrieval.
Singleton page retrieval is the most distinct modification to the attestation procedure since this interaction is introduced by \sys{}.
Thus, we expect it to dominate the overhead introduced by \sys{}.
We measured the entire time it takes to retrieve a singleton page from the verifier, as well as, the time it takes to connect to the verifier and terminate the connection again after a simple no-op request.
Figure~\ref{fig:eval:cas_interface2} shows the results of these measurements split into individual operations necessary to complete the retrieval.
We use measurements from section \S{}\ref{sec:eval:micro:sha256} to attribute the latency.
% SHA256/enclave-base-hash-finalization/4096,31406.22782855712,ns
% SigStruct/signing,4932279.035370034,ns
% SigStruct/verification-correct,408844.3005348156,ns
% CAS,Interface/open-ping-close,3737093.741232302,ns
% CAS,Interface/open-retrieve_singleton_page-close,26306670.787517827,ns
The entire operation adds about \(26.3\)\thinspace{}ms to each enclave's start.
During this operation, a negligible amount of time is spent to verify the received \gls{sigstruct}'s integrity (\(0.4\)\thinspace{}ms) and to calculate the expected singleton's enclave measurement (\(32\)\thinspace{}\(\mu{}\)s).
Establishing the connection (O/C) requires \(3.74\)\thinspace{}ms and the signing of the singleton's \gls{sigstruct} \(4.93\)\thinspace{}ms.
The majority of time is spent with miscellaneous other necessary activities in the SCONE \gls{cas}.
These involve the loading and parsing of the configuration details from the encrypted database, as well as, the enforcement of access policies.

\input{05_evaluation_macro_plots.tex}

\vspace{-2.36mm}\subsubsection*{Enclave Execution}
%In our final micro-benchmark, we evaluate the overhead \sys{} introduces for running attested \gls{sgx} enclaves in total.
We next evaluate the overhead \sys{} introduces for running attested \gls{sgx} enclaves in total.
For this benchmark, we use the minimal C program from Section~\ref{sec:eval:micro:compilation} and measure its execution time under various configurations.
We ran it in simulation mode, \ie{}, without hardware protection, with \gls{sgx} hardware protection and with hardware and attestation.
Also, we vary the enclave heap size from \(32\)\thinspace{}MB to \(2\)\thinspace{}GB.
We compare the individual measurements with each other to estimate the overheads introduced by the framework, the hardware protection and the attestation procedure.
Figure~\ref{fig:eval:execution} shows the results for \sys{} and baseline.
%e find that, throughout the benchmarks, \sys{} is slower only within single-digit microsecond values compared to the baseline for execution modes that make no use of attestation.
%Thus, we conclude that \sys{} does not introduce significant overhead to the framework's nor the hardware protection's overheads.
\sys{} is slower only within single-digit microsecond values compared to the baseline for execution modes that make no use of attestation. Thus, we conclude that \sys{} does not introduce significant overhead to the framework's nor the hardware protection's overheads.


Attestation overhead increases slightly with enclave heap size, which is an effect of increased cache pressure.
For attested execution \sys{} introduces \(132\)\thinspace{}ms to \(144.2\)\thinspace{}ms compared to \(36.3\)\thinspace{}ms to \(65.9\)\thinspace{}ms introduced by the baseline system.
Compared to the overall execution time of up to \(5.2\)\thinspace{}s (min: \(258.1\)\thinspace{}ms), these overheads are only significant in experiments with small enclave heap size.

\vspace{-3mm}\subsection{Macro-benchmarks}\label{sec:eval:macro}

In this section, we evaluate our protection mechanism overhead using real-world applications including \emph{(1)} a simple python application with an encrypted volume (Python)~\cite{python-volume}, \emph{(2)} image classification using OpenVino~\cite{openvino} (OpenVino) and \emph{(3)} Pytorch CIFAR-10 dataset training~\cite{pytorch-cifar10} (Pytorch).
%including \emph{(1)} a simple python application with an encrypted volume (Python-Vol) \cite{python-volume}, \emph{(2)} Support Vector Machine training using Sklearn library~\cite{sklearn} (Sklearn), 
We measure the duration of these workloads when running them inside \gls{sgx} enclaves with \sys{} using the SCONE attestation service \gls{cas}.
We then enable the proposed protection mechanism \sys{} in SCONE and perform the same experiments as a baseline to evaluate the impact of the protection mechanism on performance as shown in Figure~\ref{fig:macro-benchmarks}. 
\sys{} introduces \(1.03\)\%, \(2.49\)\% and \(13.2\)\% overheads with Python, Openvino, Pytorch workloads, respectively.
%\sys{} introduces \(1.03\)\%, \(2.49\)\% and \(13.2\)\% overheads in the benchmarks for Python, Openvino, Pytorch, compared to the baseline.%in comparison to the baseline.
%Our benchmarks show that for real-world applications the overhead measured during the micro-benchmarks is negligible.


==> shepherd_version/05_evaluation_macro_plots.tex <==

\begin{figure*}[!t]
    % \captionsetup{format=plain, justification=center}
	\begin{minipage}{.42\textwidth}
    % \vspace{-3pt} % vertically align the top of the figure with the fig in the left column 
    \includesvg[width=.97\textwidth]{figures/evaluation/execution2.svg}
    \caption{Measurement of program execution.}\label{fig:eval:execution}    
    \Description{No description.}
	\end{minipage}%
    \hspace{50pt}
    \begin{minipage}{.42\textwidth}
    \vspace{5pt} % vertically align the top of the figure with the fig in the left column 
    \includesvg[width=.98\textwidth]{figures/evaluation/macro-bench3_robert.svg}
    %\caption{\sys{} performance with real-world workloads.}\label{fig:macro-benchmarks}
    \caption{The performance overhead of \sys{} with real-world workloads.}\label{fig:macro-benchmarks}
    \Description{No description}
	\end{minipage}%
\end{figure*}


% \begin{figure*}[!t]
% 	\captionsetup[subfloat]{farskip=2pt,captionskip=1pt}
	
%     \subfloat[Program Execution.]
% 	{
%         \includesvg[height=.24\textwidth]{figures/evaluation/execution2.svg}\label{fig:eval:execution}
% 	}
% 	\hspace{20pt}
% 	\subfloat[Macro Benchmarks.]
% 	{
%         \includesvg[height=.24\textwidth]{figures/evaluation/macro-bench2.svg}\label{fig:macro-benchmarks}
% 	}
	
%     \caption{Micro- and Macro-Benchmarks of \sys{}}\label{fig:macro_bench}
%     \Description{No description}
% \end{figure*}

==> shepherd_version/05_evaluation_micro_plots.tex <==

\begin{figure*}[!ht]
	\captionsetup[subfloat]{farskip=2pt,captionskip=1pt}
	
    \subfloat[Compilation duration.]
	{
        \includesvg[height=.167\textwidth]{figures/evaluation/compilation.svg}\label{fig:eval:compilation}
	}
	\hspace{3pt}
	\subfloat[Sigstruct Signing and Verification.]
	{
        \includesvg[height=.163\textwidth]{figures/evaluation/sigstruct.svg}\label{fig:eval:sigstruct}
	}
	\hspace{3pt}	
	\subfloat[\sys{} operation durations.]
	{
        \includesvg[height=.167\textwidth]{figures/evaluation/t2.svg}\label{fig:eval:cas_interface2}
	}
    \caption{Micro-benchmarks of \sys{}.}\label{fig:micro_bench}
    \vspace{-2mm}
    \Description{No description}
    \rk{Improve captions!}
\end{figure*}

% \begin{figure}[t!]
%     %\vspace{3pt} % vertically align the top of the figure with the fig in the left column 
%     \centering
%     \includesvg[width=.3\columnwidth]{figures/evaluation/compilation.svg}
%     \caption{Measurement of compilation.}\label{fig:eval:compilation}
%     \Description{No description}
%     \rk{Improve Caption}
% \end{figure}


% \begin{figure}[t!]
%     %\vspace{3pt} % vertically align the top of the figure with the fig in the left column 
%     \centering
%     \includesvg[width=.3\columnwidth]{figures/evaluation/sigstruct.svg}
%     \caption{Measurement of sigstruct.}\label{fig:eval:sigstruct}
%     \Description{No description}
%     \rk{Improve Caption}
%     \rk{Improve labels in plot.}
% \end{figure}


% \begin{figure}[!t]
%     %\vspace{3pt} % vertically align the top of the figure with the fig in the left column 
%     \centering
%     \includesvg[width=.3\columnwidth]{figures/evaluation/t2.svg}
%     \caption{Measurement of the singleton page retrieval times.}\label{fig:eval:cas_interface2}
%     \Description{No description}
%     \rk{Improve Caption}
% \end{figure}


==> shepherd_version/06_related.tex <==
\vspace{-3mm}\section{Related work}

\subsubsection*{Attacks against remote attestation}
The remote attestation in several TEEs is currently vulnerable to \emph{relay attacks}.
In these attacks, an adversary can control the OS (or other software) on the target host/device to relay incoming attestation requests to another host/device.
For example, in the context of TPM attestation, the relay attack is called \emph{cuckoo attack}~\cite{parno_bootstrapping}. 
In this attack, the adversary uses malicious software on the target host to redirect the attestation to a host that he controls.
Thus, the provisioning of confidential data is directed to the host controlled by the adversary.
To handle this attack, several defense mechanisms have been proposed however they still contain several limitations~\cite{fink_catching_2011}.
For example, they require dedicated measurement conditions, e.g., turning off some OS processes. In addition, it has a high amount of false positives.

In another approach Flicker~\cite{flicker2008} attests to only a single application at the time, requiring to shut down the entire OS and all other services and also requires a trusted administrator.
Recently, several attacks against Intel \gls{sgx} remote attestation have been presented:
ProximiTEE~\cite{proximi-tee} presents a relay attack on SGX attestation, or SGAxe~\cite{van2020sgaxe} shows an attack that bypasses the SGX remote attestations.
However, these attacks require to first perform micro-ar\-chi\-tec\-tur\-al attacks such as side-channel attacks~\cite{Kocher2018spectre, chen2018sgxpectre, Foreshadow, Lipp2018meltdown}, then to use the gained secrets to attack the remote attestation. Meanwhile, we present an attack against TEEs remote attestation without requiring to perform any microarchitectural attacks.

\vspace{-2mm}\subsubsection*{Side-channel attacks}
Researchers recently demonstrated that TEEs are vulnerable to side-channel attacks~\cite{Kocher2018spectre, chen2018sgxpectre, Foreshadow, Lipp2018meltdown}.
To mitigate these attacks, protection mechanisms have been proposed~\cite{DRSGX, oblivious-ram2, oblivious-ram1, cloak, raccoon, szefer_cache_attacks}.
They follow the idea of hiding the memory access pattern of applications running inside SGX enclaves~\cite{cloak, oblivious-ram2, oblivious-ram1, DRSGX} by generating random memory accesses or shuffling the encrypted memory elements in a way that the observable access patterns are similar to each other and independent from the original access patterns.
%Intel has been also working to release various patches, microcode updates to mitigate SGX side-channel attacks. 
In this paper, We however turn our focus to the second key feature of \glspl{tee}, which is the \emph{remote attestation} mechanism.
We present an attack that bypasses the remote attestation protocol. Our attack does not require attacking the sealing mechanism of TEEs as the previous work~\cite{van2020sgaxe}. 
%Mentioned in attack:
%Our attack does not require attacking the sealing mechanism of TEEs as the previous work~\cite{van2020sgaxe}.  

\vspace{-2mm}\subsubsection*{Support legacy applications} 
To support legacy applications running with Intel \gls{sgx} without changing their source code, several SGX platforms~\cite{arnautov2016scone, priebe2019sgx, tsai2017graphene, shen2020occlum} have been developed and are used in practice.
SCONE~\cite{arnautov2016scone} was the first framework that supported switchless system calls to improve the performance of applications running with Intel SGX.
Following this idea, other SGX frameworks such as Graphene-SGX~\cite{tsai2017graphene}, SGX-LKL~\cite{priebe2019sgx} or Occlum~\cite{shen2020occlum} were proposed.
%Unfortunately, Graphene-SGX~\cite{tsai2017graphene} and Occlum~\cite{occlum} only provide the building blocks for users to perform remote attestation and secret provisioning for their applications.
Among these frameworks, only SCONE and SGX-LKL support a transparently performing remote attestation mechanism for users.
However, in this paper, we demonstrate that the supported mechanism is not secure by showing an attack to bypass the remote attestation.
We also provide novel protection against this attack and strengthen the remote attestation mechanism of SCONE with only lightweight overhead. 
%{\bf Occlum~\cite{shen2020occlum}}
%Occlum is a multi-process library OS for Intel SGX.
%The Occlum platform abstraction layer utilizes Intel's SGX SDK to create enclaves.
%Each Occlum instance is built from an identical library OS shared object.
%However, for each application (or workspace) the shared object is updated with the MAC of the application specific Occlum configuration file.
%This file contains, among others, the protection information of the files in the file system.
%% The mac is included via `objcopy --update-section .builtin_config=temp_mac_file libocclum-libos.so' and the mrenclave is
%% calculated with the Intel SDK signer tool running across that very .so. TODO: Does the signer consider all sections?
%
%{\bf Asylo} 
%Uses the Intel-SDK underneath. No real paper available, just the website.
%
%{\bf Intel SGX~\cite{costan2016intel}}
%
%{\bf OpenEnclave~\cite{openenclave}}
%
%{\bf SGX-LKL~\cite{priebe2019sgx}}
%
%{\bf ENARX~\cite{enarx}}
%
%{\bf Graphene-SGX~\cite{tsai2017graphene}}
%
%Graphene-SGX is a library \gls{os} that supports executing of legacy applications inside of \gls{sgx} enclaves.
%In Graphene-SGX, application and the files their accessing are described in a \textit{manifest} file.


%{\bf Dynamic Integrity Measurement}
%With dynamic integrity measurement and attestation, as proposed in~\cite{davi2009dynamic}, the runtime state of a program is shown to challengers.

% {\bf Attacks against Intel SGX}. 
% \emph{ Side-channel attacks}
% SGX protects and ensures the confidentiality and integrity of code and data inside enclaves. Unfortunately, it still contains several practical limitations~\cite{ side channel attack works, Dark-ROP}. Recently, it has been shown that attackers can observe side channels to reveal large amounts of sensitive information of applications running insides enclaves~\cite{side channel attack works}. Controlled-channel attacks trigger page faults to observe memory access patterns to break the confidentiality of a enclave~\cite{}. Cache side channels attacks exploit the caching mechanism of CPUs as the cache layer can be shared among processes~\cite{}.   In addition, recently, speculative attacks~\cite{} make use of the side channels as a way of retrieving sensitive information.
% In general, these side-channel attacks need to interrupt the enclave frequently using a malicious kernel. As a result, the straightforward way to handle these attacks are to detect or avoid enclave interruptions~\cite{T-SGX, Dejavu}. Varys~\cite{varys-atc2018} takes a pragmatic approach of strict reservation of physical cores to security sensitive threads, thereby preventing the attacker from accessing shared CPU resources during enclave execution.
% Recently,  an attack obtained memory access pattern at the page level without triggering any page fault  has been proposed. To protect against this attack, we need a mechanism to hide the memory access patterns. DR.SGX~\cite{} proposed a mechanism to perform a fine-grained randomization at cache line level. Oblivious mechanisms have been not only applied to  cache-channel but also other channels~\cite{Opaque}. 

% {\bf Attacks from insides enclaves} Beside side-channel attacks, the code inside enclaves may have vulnerabilities which allow attackers to exploit to take control over the application during runtime. 
% Multiple works have adopted return-oriented programming (ROP)  to perform code-reuse attacks against enclaves~\cite{ROP, Dark-ROP, ...}. Typically, the ROP-based attack can be mitigated using the mechanism introduced in Haven~\cite{} and VC3~\cite{} which integrate a symmetrically encrypted enclave with a loader to receive the secret via remote attestation. The secret only can be obtained within an enclave after the remote attestation. 
% Dark-ROP~\cite{} makes use not only ROP but also several oracles which reports the internal status of enclave execution. Dark-ROP reuses code snippets called gadgets to undermine non-executable memory protection. Dark-ROP extracts the secrets by crashing and reconstructing enclaves multiple time while preserving the memory layout. To perform the Dark-
% ROP attack, it requires a non-randomized memory layout. Thus, SGX-Shield mitigated this attack by implementing SGX randomization which change the memory layout everytime a enclave is created. In this paper, we show that …


%{\bf Function as a service}
%\glsreset{faas}
%\gls{faas} or serverless is a cloud paradigm in which the user only contributes their code while the cloud operator provides all infrastructure.
%This delegates more responsibilities to the cloud operator as done in \gls{iaas} in which the user builds their application with infrastructural build blocks offered by the cloud operator, but it still allows the user to run their own code, which isn't the case with \gls{saas} anymore.
%In \gls{faas}, cloud operators have complete control over the scheduling of user code.
%For example, they might retire a user's program entirely when not used making more efficient of compute and memory resources.
%
%Works that protect faas with sgx: \cite{trach2019clemmys}, \cite{alder2019s}, \cite{brenner2019trust}, \cite{qiang2018se}
%


%\subsection{Enclave Caching}
%% Might be of interest: %
%The Enclave Cache Pool Management (EPM) (\url{https://github.com/alibaba/inclavare-containers/blob/master/docs/design/epm/design.md}) is a service that decouples enclave creation from their use.
%Enclaves are created at an earlier time such that when needed they can be used instantly (507ms vs. 22ms).
%Without singleton enclaves the user cannot ensure that the enclave they're using was not tampered before.


==> shepherd_version/06_related_big_picture.tex <==
\section{RELATED WORK}

{\bf Occlum~\cite{shen2020occlum}}
Occlum is a multi-process library OS for Intel SGX.
The Occlum platform abstraction layer utilizes Intel's SGX SDK to create enclaves.
Each Occlum instance is built from an identical library OS shared object.
However, for each application (or workspace) the shared object is updated with the MAC of the application specific Occlum configuration file.
This file contains, among others, the protection information of the files in the file system.
% The mac is included via `objcopy --update-section .builtin_config=temp_mac_file libocclum-libos.so' and the mrenclave is
% calculated with the Intel SDK signer tool running across that very .so. TODO: Does the signer consider all sections?

{\bf Asylo} 
Uses the Intel-SDK underneath. No real paper available, just the website.

{\bf Intel SGX~\cite{costan2016intel}}

{\bf OpenEnclave~\cite{openenclave}}

{\bf SGX-LKL~\cite{priebe2019sgx}}

{\bf ENARX~\cite{enarx}}

{\bf Graphene-SGX~\cite{tsai2017graphene}}

Graphene-SGX (now it is changed to Gramine~\cite{Gramine}}) is a library \gls{os} that supports executing of legacy applications inside of \gls{sgx} enclaves.
In Graphene-SGX, application and the files their accessing are described in a \textit{manifest} file.


{\bf Dynamic Integrity Measurement}
With dynamic integrity measurement and attestation, as proposed in~\cite{davi2009dynamic}, the runtime state of a program is shown to challengers.

% {\bf Attacks against Intel SGX}. 
% {\em Side-channel attacks}
% SGX protects and ensures the confidentiality and integrity of code and data inside enclaves. Unfortunately, it still contains several practical limitations~\cite{ side channel attack works, Dark-ROP}. Recently, it has been shown that attackers can observe side channels to reveal large amounts of sensitive information of applications running insides enclaves~\cite{side channel attack works}. Controlled-channel attacks trigger page faults to observe memory access patterns to break the confidentiality of a enclave~\cite{}. Cache side channels attacks exploit the caching mechanism of CPUs as the cache layer can be shared among processes~\cite{}.   In addition, recently, speculative attacks~\cite{} make use of the side channels as a way of retrieving sensitive information.
% In general, these side-channel attacks need to interrupt the enclave frequently using a malicious kernel. As a result, the straightforward way to handle these attacks are to detect or avoid enclave interruptions~\cite{T-SGX, Dejavu}. Varys~\cite{varys-atc2018} takes a pragmatic approach of strict reservation of physical cores to security sensitive threads, thereby preventing the attacker from accessing shared CPU resources during enclave execution.
% Recently,  an attack obtained memory access pattern at the page level without triggering any page fault  has been proposed. To protect against this attack, we need a mechanism to hide the memory access patterns. DR.SGX~\cite{} proposed a mechanism to perform a fine-grained randomization at cache line level. Oblivious mechanisms have been not only applied to  cache-channel but also other channels~\cite{Opaque}. 

% {\bf Attacks from insides enclaves} Beside side-channel attacks, the code inside enclaves may have vulnerabilities which allow attackers to exploit to take control over the application during runtime. 
% Multiple works have adopted return-oriented programming (ROP)  to perform code-reuse attacks against enclaves~\cite{ROP, Dark-ROP, ...}. Typically, the ROP-based attack can be mitigated using the mechanism introduced in Haven~\cite{} and VC3~\cite{} which integrate a symmetrically encrypted enclave with a loader to receive the secret via remote attestation. The secret only can be obtained within an enclave after the remote attestation. 
% Dark-ROP~\cite{} makes use not only ROP but also several oracles which reports the internal status of enclave execution. Dark-ROP reuses code snippets called gadgets to undermine non-executable memory protection. Dark-ROP extracts the secrets by crashing and reconstructing enclaves multiple time while preserving the memory layout. To perform the Dark-
% ROP attack, it requires a non-randomized memory layout. Thus, SGX-Shield mitigated this attack by implementing SGX randomization which change the memory layout everytime a enclave is created. In this paper, we show that …


{\bf Function as a service}
\glsreset{faas}
\gls{faas} or serverless is a cloud paradigm in which the user only contributes their code while the cloud operator provides all infrastructure.
This delegates more responsibilities to the cloud operator as done in \gls{iaas} in which the user builds their application with infrastructural build blocks offered by the cloud operator, but it still allows the user to run their own code, which isn't the case with \gls{saas} anymore.
In \gls{faas}, cloud operators have complete control over the scheduling of user code.
For example, they might retire a user's program entirely when not used making more efficient of compute and memory resources.

Works that protect faas with sgx: \cite{trach2019clemmys}, \cite{alder2019s}, \cite{brenner2019trust}, \cite{qiang2018se}

{\bf Side-channel attacks}
Researchers recently demonstrated that TEEs  are vulnerable to side-channel attacks~\cite{Kocher2018spectre, chen2018sgxpectre, Foreshadow, Lipp2018meltdown}. To mitigate these attacks, protection mechanisms have been proposed~\cite{DRSGX, oblivious-ram2, oblivious-ram1, cloak,  raccoon, szefer_cache_attacks}. Intel has been also working to release various patches, microcode updates to mitigate SGX side-channel attacks.
In this paper, we however turn our focus to the second key feature of TEEs which is the {\em remote attestation} mechanism.  We present an attack that bypasses the remote attestation protocol. Our attack does not require attacking the sealing mechanism of TEEs as the previous work~\cite{van2020sgaxe}.  

\subsection{Enclave Caching}
% Might be of interest: %
The Enclave Cache Pool Management (EPM) (\url{https://github.com/alibaba/inclavare-containers/blob/master/docs/design/epm/design.md}) is a service that decouples enclave creation from their use.
Enclaves are created at an earlier time such that when needed they can be used instantly (507ms vs. 22ms).
Without singleton enclaves the user cannot ensure that the enclave they're using was not tampered before.

==> shepherd_version/07_conclusion.tex <==
% Not part of this paper anymore.
% The underlying thoughts here should be moved into a paragraph of the discussion/conclusion.

% \section{A PUBLIC CONFIGURATION INTERFACE}

% Up until now we assumed that the \gls{tee} program's behavior is mostly determined by its configuration as it is the case for instance for language interpreters.
% In this section we'll lift that assumption arguing that most non-trivial programs are vulnerable taking Redis as an example.

% \subsection{Going through the backdoor}
% We observe that most legacy software is developed as if its configuration and data is benign.
% Therefore, we suspect code handling configuration and data to be less robust to manipulations compared to code handling data from potentially hostile sources, such as the network.
% When such software is execute under a \gls{tee} suitable threat model, however, the attacker can easily manipulate configuration and data to mount an attack.
% Their goal would be to hijack the program's control flow to produce an \gls{sgx} report.
% The necessary instruction to produce the report have to be in the binary already as the program itself, if executed in a \gls{tee}, would want to engage in remote attestation.
% Along these lines, we hypothesis that even well tested, productive software is exploitable under the \gls{tee} threat model.

% To test our assumption we searched for exploitable code in Redis.
% Redis is a key-value database that was first published in 2009.
% It is popular in the industry: in the DB-Engines key-value stores popularity ranking it takes the first place and on Docker Hub it the fifth most downloaded image.
% Due to its widespread usage, we assume, Redis is well-vetted and found vulnerabilities are closed in a timely fashion.

% Redis obtains its configuration via command line arguments and an configuration file.
% The configuration options are extensive.
% Among them is the path of the database dump file.
% The database dump file stores key-value data in a binary format on disk for persistence.
% \fg{TODO add figure of Redis Architecture}

% To find a suitable vulnerability to hijack the control flow we used \gls{afl} to fuzz the Redis database dump file.
% During the fuzzing, \gls{afl} repeatably manipulates a database dump file and observes the application's behavior when it is started with the manipulated file.
% If it crashes with a page fault, chances are high that the manipulation of the dump file leads to an exploitable memory corruption in Redis.
% We found hundreds of manipulations that lead to crashes.
% Upon further investigation we found a code pattern (Listing X) that can be used to hijack control flow through \gls{rop}. \fg{TODO: add Listing}
% In this piece of code, data from the database dump file is copied onto the stack into an array of 128 bytes length.
% However, the size of the \texttt{memcpy} instruction is read from the dump file as well without consideration of the fixed length of copy's destination.
% Therefore, any data copied beyond the reserved 128 bytes overwrites the stack enabling \gls{rop}.
% \gls{rop} has already shown to be effective against \gls{sgx}~\cite{biondo2018guard, lee2017hacking}.

% To mount the whole attack, an adversary would first analyze the binary for the necessary \gls{rop} gadgets and use this information to manufacture a malicious database dump file that would exploit the found vulnerability to produce the required \gls{sgx} report and provide it to the attacker.
% They would then package the malicious dump file such that the SGX framework would reproduce the victim environment, \eg, with SGX-LKL it would have to be put into an encrypted file system image and start it using the frameworks attestation and configuration method to trigger the loading of the prepared dump file within the correct setup \gls{tee}.
% This would produce the necessary attestation report which can be used to obtain the victim's secrets as discussed in Section~\ref{}.

% \subsection{A Simpler Approach}
% \fg{TODO: What about applications with plugins that are dynamic libraries loaded at runtime? e.g. PCSCD}

\section{Conclusion}
In this paper, we show that the measurement for remote attestation in TEEs is currently vulnerable to certain ``resue'' attacks of enclaves since it only guarantees software integrity before it runs, but not during runtime.
We demonstrate a such practical attack against different TEE frameworks. 
In addition, we provide a solution to strengthen the measurement by considering all aspects that determine the behavior of remote applications and ensure the measurement is fresh. 
We evaluate our protection mechanism with real-world applications. 
The evaluation shows that it can protect against reuse attacks and incurs only negligible overhead. %which is only from $1.03$\% to $13.2$\% depending on running applications.

\small
\vspace{-1mm}\subsubsection*{Acknowledgements}
% We thank our reviewers and our shepherd Valerio Schiavoni for their work.
We thank Andrey Brito, our reviewers, and our shepherd Valerio Schiavoni for their work.
% Cloudskin: 101092646
% Neardata: 101092644 
% AI-Sprint: 101016577
% 6G-Life: BMBF (Federal Ministry of Education and Research)
This publication was funded by the European Union's Horizon Europe
research and innovation program under grant agreements 101092646 (Cloudskin), 101016577 (Neardata), 101092644 (AI-Sprint), by the Deutsche Forschungsgemeinschaft (DFG) in subproject B07 of the Collaborative Research Center Transregio 96 (project 174223256), and by the Federal Ministry of Education and Research (6G-Life).
\normalsize

==> shepherd_version/mac.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% mac.tex
%%
%% Umut A. Acar
%% Macros for adaptive computation paper.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\readarrow}{\ensuremath{\Longrightarrow}}
\newcommand{\currenttime}{\ttt{currentTime}\xspace}
\newcommand{\tags}[1]{\ensuremath{\mathsf{tags}(#1)}}
\newcommand{\weight}[1]{\ensuremath{\mathsf{weight}(#1)}}
\newcommand{\dist}[2]{\ensuremath{\delta(#1,#2)}}


\newcommand{\cutspace}{\vspace{-4mm}}

\newcommand{\bomb}[1]{\fbox{\mbox{\emph{\bf {#1}}}}}

\newcommand{\myparagraph}[1]{\smallskip{}\noindent{\bf{}{#1}.\hspace{.2em}}\nopagebreak{}}
\newcommand{\tightparagraph}[1]{\noindent{\bf{}{#1}.\hspace{.2em}}\nopagebreak{}}
\newcommand{\subheading}[1]{\vspace{2mm}\noindent{\bf{}{#1}}\\\noindent{}}
% formatting stuff
\newcommand{\codecolsep}{1ex}



\newcommand{\rlabel}[1]{\hspace*{-1mm}\mbox{\small{\bf ({#1})}}}

\newcommand{\tablerow}{\\[5ex]}
\newcommand{\tableroww}{\\[7ex]}
\newcommand{\tableline}{
\vspace*{2ex}\\
\hline\\ 
\vspace*{2ex}}

% Don't care
\newcommand{\dontcare}{\_
}

%% Comment sth out. 
\newcommand{\out}[1] {}
\newcommand{\sthat}{\ensuremath{~|~}}

%% definitions
\newcommand{\defi}[1]{{\bfseries\itshape #1}}

% Code listings.
\newcounter{codeLineCntr}
\newcommand{\codeLine}
 {\refstepcounter{codeLineCntr}{\thecodeLineCntr}}
\newcommand{\codeLineL}[1]
 {\refstepcounter{codeLineCntr}\label{#1}{\thecodeLineCntr}}
\newcommand{\codeLineNN}{} %% NN = No-Number (and no change to counter)

\newenvironment{codeListing}
 {\setcounter{codeLineCntr}{0}
%  \fontsize{10}{12}
 % the first one is width the second is height
 \fontsize{9}{11}
  \fontsize{8}{8}
  \vspace{-.1in}
  \ttfamily\begin{tabbing}}
  {\end{tabbing}
   \vspace{-.1in}}

\newenvironment{codeListing8}
 {\setcounter{codeLineCntr}{0}
%  \fontsize{8}{10}
  \fontsize{8}{8}
  \vspace{-.1in}
  \ttfamily
  \begin{tabbing}}
 {\end{tabbing}
 \vspace{-.1in}
}

\newenvironment{codeListing8h}
 {\setcounter{codeLineCntr}{0}
  \fontsize{8.5}{10.5}
  \vspace{-.1in}
  \ttfamily
  \begin{tabbing}}
 {\end{tabbing}
 \vspace{-.1in}
}


\newenvironment{codeListing9}
 {\setcounter{codeLineCntr}{0}
  \fontsize{9}{11}
  \vspace{-.1in}
  \ttfamily
  \begin{tabbing}}
 {\end{tabbing}
 \vspace{-.1in}
}

\newenvironment{codeListing10}
 {\setcounter{codeLineCntr}{0}
  \fontsize{10}{12}
  \vspace{-.1in}
  \ttfamily
  \begin{tabbing}}
 {\end{tabbing}
 \vspace{-.1in}
}


\newenvironment{codeListingNormal}
 {\setcounter{codeLineCntr}{0}
  \vspace{-.1in}
  \ttfamily
  \begin{tabbing}}
 {\end{tabbing}
 \vspace{-.1in}
}

\newcommand{\codeFrame}[1]
{\begin{center}\fbox{\parbox[t]{\columnwidth}{#1}}\end{center}
% \vspace*{-.15in}
}

\newcommand{\halfBox}[1]
{\begin{center}\fbox{\parbox[t]{\columnwidth}{#1}}\end{center}
% \vspace*{-.15in}
}

\newcommand{\fullBox}[1]
{\begin{center}\fbox{\parbox[t]{\textwidth}{#1}}\end{center}
% \vspace*{-.15in}
}

%%Note this is redefined in local-mac.tex for each paper.
\newcommand{\fixedCodeFrame}[1]
{
\begin{center}
\fbox{
\parbox[t]{0.9\columnwidth}{
#1
}
}\end{center}
}

% Footnote commands.
\newcommand{\footnotenonumber}[1]{{\def\thempfn{}\footnotetext{#1}}}

% Margin notes - use \notesfalse to turn off notes.
\setlength{\marginparwidth}{0.6in}
\reversemarginpar
\newif\ifnotes
\notestrue
\newcommand{\longnote}[1]{
  \ifnotes
    {\medskip\noindent Note:\marginpar[\hfill$\Longrightarrow$]
      {$\Longleftarrow$}{#1}\medskip}
  \fi}
\newcommand{\note}[1]{
  \ifnotes
    {\marginpar{\raggedright{\tiny #1}}}
  \fi}
\newcommand{\notered}[1]{\ifnotes
    {\marginpar{\raggedright{\tiny
          {\sf\color{red} #1}}}}
    \fi}


% Stuff not wanted.
\newcommand{\punt}[1]{}

% Sectioning commands.
\newcommand{\subsec}[1]{\subsection{\boldmath #1 \unboldmath}}
\newcommand{\subsubheading}[1]{\paragraph*{#1}}



\newcommand{\partref}[1]{Part~\ref{part:#1}}
\newcommand{\chref}[1]{Chapter~\ref{ch:#1}}
\newcommand{\chreftwo}[2]{Chapters \ref{ch:#1} and~\ref{ch:#2}}
\newcommand{\chrefthree}[3]{Chapters \ref{ch:#1}, and~\ref{ch:#2}, and~\ref{ch:#3}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Subsection~\ref{subsec:#1}}
\newcommand{\secreftwo}[2]{Sections \ref{sec:#1} and~\ref{sec:#2}}
\newcommand{\secrefthree}[3]{Sections \ref{sec:#1},~\ref{sec:#2},~and~\ref{sec:#3}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\figreftwo}[2]{Figures \ref{fig:#1} and~\ref{fig:#2}}
\newcommand{\figrefthree}[3]{Figures \ref{fig:#1}, \ref{fig:#2} and~\ref{fig:#3}}
\newcommand{\figreffour}[4]{Figures \ref{fig:#1},~\ref{fig:#2},~\ref{fig:#3}~and~\ref{fig:#4}}
\newcommand{\figpageref}[1]{page~\pageref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\tabreftwo}[2]{Tables~\ref{tab:#1} and~\ref{tab:#1}}

\newcommand{\stref}[1]{step~\ref{step:#1}}
\newcommand{\caseref}[1]{case~\ref{case:#1}}
\newcommand{\lineref}[1]{line~\ref{line:#1}}
\newcommand{\linereftwo}[2]{lines \ref{line:#1} and~\ref{line:#2}}
\newcommand{\linerefthree}[3]{lines \ref{line:#1},~\ref{line:#2},~and~\ref{line:#3}}
\newcommand{\linerefrange}[2]{lines \ref{line:#1} through~\ref{line:#2}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\thmreftwo}[2]{Theorems \ref{thm:#1} and~\ref{thm:#2}}
\newcommand{\thmrefthree}[3]{Theorems \ref{thm:#1}, \ref{thm:#2} and~\ref{thm:#3}}
\newcommand{\thmpageref}[1]{page~\pageref{thm:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\lemreftwo}[2]{Lemmas \ref{lem:#1} and~\ref{lem:#2}}
\newcommand{\lemrefthree}[3]{Lemmas \ref{lem:#1},~\ref{lem:#2},~and~\ref{lem:#3}}
\newcommand{\lempageref}[1]{page~\pageref{lem:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\defreftwo}[2]{Definitions \ref{def:#1} and~\ref{def:#2}}
\newcommand{\defpageref}[1]{page~\pageref{def:#1}}
\renewcommand{\eqref}[1]{Equation~(\ref{eq:#1})}
\newcommand{\eqreftwo}[2]{Equations (\ref{eq:#1}) and~(\ref{eq:#2})}
\newcommand{\eqpageref}[1]{page~\pageref{eq:#1}}
\newcommand{\ineqref}[1]{Inequality~(\ref{ineq:#1})}
\newcommand{\ineqreftwo}[2]{Inequalities (\ref{ineq:#1}) and~(\ref{ineq:#2})}
\newcommand{\ineqpageref}[1]{page~\pageref{ineq:#1}}
\newcommand{\itemref}[1]{Item~\ref{item:#1}}
\newcommand{\itemreftwo}[2]{Item~\ref{item:#1} and~\ref{item:#2}}

% Useful shorthands.
\newcommand{\abs}[1]{\left| #1\right|}
\newcommand{\card}[1]{\left| #1\right|}
\newcommand{\norm}[1]{\left\| #1\right\|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
  \renewcommand{\choose}[2]{{{#1}\atopwithdelims(){#2}}}
\newcommand{\ang}[1]{\langle#1\rangle}
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\prob}[1]{\Pr\left\{ #1 \right\}}
\newcommand{\expect}[1]{\mathrm{E}\left[ #1 \right]}
\newcommand{\expectsq}[1]{\mathrm{E}^2\left[ #1 \right]}
\newcommand{\variance}[1]{\mathrm{Var}\left[ #1 \right]}
\newcommand{\twodots}{\mathinner{\ldotp\ldotp}}

% Standard number sets.
\newcommand{\reals}{{\mathrm{I}\!\mathrm{R}}}
\newcommand{\integers}{\mathbf{Z}}
\newcommand{\naturals}{{\mathrm{I}\!\mathrm{N}}}
\newcommand{\rationals}{\mathbf{Q}}
\newcommand{\complex}{\mathbf{C}}

% Special styles.
\newcommand{\proc}[1]{\ifmmode\mbox{\textsc{#1}}\else\textsc{#1}\fi}
\newcommand{\procdecl}[1]{
  \proc{#1}\vrule width0pt height0pt depth 7pt \relax}
  \newcommand{\func}[1]{\ifmmode\mathrm{#1}\else\textrm{#1}fi} %
%  Multiple cases.  
\renewcommand{\cases}[1]{\left\{
  \begin{array}{ll}#1\end{array}\right.}
  \newcommand{\cif}[1]{\mbox{if $#1$}} 

%% spacing hacks
\newcommand{\longpage}{\enlargethispage{\baselineskip}}
\newcommand{\shortpage}{\enlargethispage{-\baselineskip}}



==> shepherd_version/rebuttal.tex <==
Our response
We would like to express our sincere gratitude for your valuable feedback.

Reviewer A, Unclear parts in Section 3 and Section 4
The reviewer mentioned that it’s not clear which part in Figure 4 belongs to the attacker. We indicated the parts in red color are untrusted parts, e.g., under the control of the attacker. We will indicate clearly "TEE impersonator" and "report server" components in Figure 4 in the revised version.

Reviewer A, No detailed information in the implementation of the proposed solution
In fact, in Section 3.3 we present the implementation of the attack and in Section 4.4 we present our solution together on how to implement it with Intel SGX. We can make it more clear in the revised version.

Reviewer A, Concerns about the future of Intel SGX
In the confidential computing summit 2023, Intel announced that Intel SGX and Intel TDX will co-exist, and Intel will provide hardware that has both SGX and TDX functionalities. SGX focuses on protecting at the process level meanwhile TDX focuses on the VM level. This vulnerability described in our paper has been discussed with Intel.


Reviewer A Reviewer B,  how to extend the work for Intel TDX or alternative TEEs
AMD SEV and Intel TDX offer confidential encrypted VMs to users. They have a similar issue since these TEEs only perform measurements and ensure the integrity of the VMs after the booting process. During computation, these TEEs do not perform any measurements if shared data or libraries from the host are loaded to the VMs, it requires carefully checking or adding their measurement during the boot process. If there is no shared data or libraries between VMs or with the host, an attacker can just boot the VM from a victim and perform, e.g., side-channel attacks on the VM in a lab environment. The goal of the proposed protection mechanism is to allow users to create a singleton SGX enclave that can be extended to a singleton confidential VM. In the singleton confidential VM, the measurement process during booting time includes the user identity and security for that VM. In other words, an attacker cannot just boot a VM of the user since he/she cannot generate the unique measurement of the VM. Only after verifying that the VM is an unique single instance, secrets are injected in the VM. 

Reviewer C, the attacks can be prevented using statically linking
Technically, yes. However, it requires users to recompile their applications, for interpreter languages like Python, and Java, they need to pack dependencies with interpreter engines which is cumbersome, and requires heavy engineering, especially with complex libraries such as TensorFlow. 
It also comes with the cost of increased binary size which makes booting time slow,  compatibility issues, performance overhead, and resource redundancy.

Reviewer D, not clear how the attacker would intercept the attestation process
The attacker does not intercept the attestation process but bypasses the process. The remote attestation process only performs measurement of the binary of the application when it is loaded into an enclave. For interpreter languages e.g., Python, the process just measures only the Python interpreter engine, it will be the same for all Python applications. Thus an attacker can just bypass it since it has the same Python interpreter engine as the victims and is running his malicious Python application on the same physical host as the victims. After the attestation process, the verifier or a Key Management System will provide secrets (keys to decrypt input data) to the Python enclave, and attackers can just get the keys using their malicious code embedded inside a library which is loaded during runtime.  We make it more clear in the revised version.

Reviewer D, Too strong assumption for the attack
Reviewer D mentioned that the adversary controls the machine during enclave initialization time, which is a strong assumption. The assumption is the same with the threat model of Intel SGX, in which attackers have privileged access, e.g., root access. The input data and code are typically encrypted before uploading them to an untrusted host. Thus, attackers with root access cannot just read the code and data.

Reviewer D, why the solution Haven is not secure
Yes, the Haven system incorporates configurations into the TEE such that the attestation would also include them. This would also reveal the TEE’s configuration and, thus, its secrets because the configurations are in plaintext in the file system before loading inside TEE.



==> shepherd_version/security_argument.tex <==
\section{Security Argument}

In this section we will highlight the important of attestation for the secure usage of \gls{sgx} enclaves and point out where it falls short in protecting dynamic applications.

The threat-model of \gls{sgx} offers the adversary many points to manipulate an enclave.
For example, the enclave might be manipulated at rest, during transmission or at construction time.
After the enclave has been initializes, however, it is protected by the processor from any further manipulation from outside the enclave itself.
Consequently, before trusting an enclave the user must ensure themselves that it was constructed according to their expectations.

Therefore, \gls{sgx} enables the enclave to create a \gls{sgx} report that describes the enclave's state during initialization.
Updates to the enclave after its initialization do not effect the generated report.
This report can be verified by an other enclave on the same platform in a procedure known as local attestation.
For this paper the details of this procedure, as well as the details of the subsequent remote attestation procedure are of little importance.
The report's body is integrity protected with a hash keyed MAC.
It includes a field of 64~bytes length that can be filled with arbitrary data, the \texttt{reportdata} field.
This field is most often used to bind some enclave chosen data to the enclave's report proving the enclave owns the data.
During the start of a configurable enclave, this data will most likely contain some key material that can be used to sent the enclave configuration data or establish a secure channel to it to do so.
Other times it might bind some result produced by the enclave.
Thus, an enclave's report can be used to proof that there is some enclave running with a certain code and signer identity.
The assumption is that the behavior of the enclave is entirely determined through its initial code and signer.

In practice, however, this is often not the case as most non-trivial programs allow modification of their behavior through configuration or data and code dynamically loaded at runtime.
Most program's behavior can be configured through environment variables or program arguments.
For interpreted or byte-code languages (Python, JavaScript, Java, ...), the initial enclave state is most likely only the language interpreter while the actual program code is read from the file system.
In \gls{faas} systems, user code is dynamically dispatched to an engine that is often started beforehand

==> shepherd_version/space-tricks.tex <==
% -*- root: main.tex -*-

%space left between floats.
\setlength{\floatsep}{4mm}
% space between last top float or first bottom float and the text.
\setlength{\textfloatsep}{2mm}

% space left on top and bottom of an in-text float.
\setlength{\intextsep}{0.5mm}


% This has the largest impact:
% space above caption
\setlength{\abovecaptionskip}{9pt}


%space below caption
\setlength{\belowcaptionskip}{0mm}

%% Change figure handling
\renewcommand{\topfraction}{0.9}
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{1}



\usepackage[inline]{enumitem}
\setlist{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}

%\usepackage[subtle]{savetrees}
% \usepackage[moderate]{savetrees}

\usepackage{setspace}
\usepackage[margin=5pt,font={stretch=0.9}]{caption}
%\usepackage[margin=8pt,font={small,bf,stretch=0.85}]{caption}


%\usepackage[small,compact,noindentafter]{titlesec}
%\usepackage[compact]{titlesec}
%
%\titlespacing\section{0pt}{6pt plus 2pt minus 2pt}{2pt plus 2pt minus 2pt}
%\titlespacing\subsection{0pt}{4pt plus 2pt minus 2pt}{2pt plus 1pt minus 1pt}
%\titlespacing{\paragraph}{0pt}{2pt plus 0pt minus 1pt}{1.0ex}
%

